Bypassing Logits Bias in Online Class-Incremental Learning with a Generative Framework

Continual learning requires the model to maintain the learned knowledge while learning from a non-i.i.d data stream continually. Due to the single-pass training setting, online continual learning is very challenging, but it is closer to the real-world scenarios where quick adaptation to new data is appealing. In this paper, we focus on online class-incremental learning setting in which new classes emerge over time. Almost all existing methods are replay-based with a softmax classifier. However, the inherent logits bias problem in the softmax classifier is a main cause of catastrophic forgetting while existing solutions are not applicable for online settings. To bypass this problem, we abandon the softmax classifier and propose a novel generative framework based on the feature space. In our framework, a generative classifier which utilizes replay memory is used for inference, and the training objective is a pair-based metric learning loss which is proven theoretically to optimize the feature space in a generative way. In order to improve the ability to learn new data, we further propose a hybrid of generative and discriminative loss to train the model. Extensive experiments on several benchmarks, including newly introduced task-free datasets, show that our method beats a series of state-of-the-art replay-based methods with discriminative classifiers, and reduces catastrophic forgetting consistently with a remarkable margin.

==> conference_101719.tex <==
%\documentclass[conference]{IEEEtran}
\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{times}
\usepackage{soul}
\usepackage{url}
\usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{amstex}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}
\urlstyle{same}
\usepackage{bm}
\usepackage{mathtools}
% the following package is optional:
%\usepackage{latexsym}
\usepackage{color}
\usepackage{amsfonts} % Use the postscript times font!
\usepackage{amsmath}
%\usepackage{soul}
\usepackage{url}
%\usepackage[hidelinks]{hyperref}
\usepackage[utf8]{inputenc}
%\usepackage[small]{caption}
\usepackage[switch]{lineno}

%\def\propositionautorefname{Proposition}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subfig}
\usepackage{algorithm}
\usepackage{algorithmic}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\begin{document}

\title{Bypassing Logits Bias in Online Class-Incremental Learning with a Generative Framework\\

}


\author{\IEEEauthorblockN{Anonymous Authors}}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to \LaTeX{} to determine where to break
% the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% puts 3 of 4 authors names on the first line, and the last on the second
% line, try using \AND instead of \And before the third author name.

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

%\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
%\newcommand{\cite}[1]{\citeauthor{#1} \shortcitep{#1}} 
%\newcommand{\cite}{\cite} 



% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\def\memory{\mathcal{M}}
\def\newbatch{\mathcal{B}_n}
\def\replaybatch{\mathcal{B}_r}
\def\tt{\bm \theta}
\def\x{\bm x}
\def\logit{\bm o}
\def\z{\bm z}
\def\y{\bm y}
\def\t{\bm t}
\def\c{\bm c}
\def\p{\bm p}
\def\haty{\hat{\bm y}}
%\newcommand{\Scos}{S^{\text{cos}}}
\newcommand{\Scos}{S}
\def\xi{{\bm x}_i}
\def\zi{{\bm z}_i}
\def\yi{{\bm y}_i}
\def\yc{{\bm y}_c}
\def\bmu{{\boldsymbol{\mu}}}
\def\D{\mathcal{D}}
\newcommand{\ceq}{\stackrel{\mathclap{\normalfont\mbox{c}}}{=}}
\newcommand{\capprox}{\stackrel{\mathclap{\normalfont\mbox{c}}}{\approx}}
\newcommand{\cleq}{\stackrel{\mathclap{\normalfont\mbox{c}}}{\leq}}
\newcommand{\cgeq}{\stackrel{\mathclap{\normalfont\mbox{c}}}{\geq}}


\maketitle

\begin{abstract}
Continual learning requires the model to maintain the learned knowledge while learning from a non-i.i.d data stream continually. Due to the single-pass training setting, online continual learning is very challenging, but it is closer to the real-world scenarios where quick adaptation to new data is appealing. In this paper, we focus on \textit{online class-incremental learning} setting in which new classes emerge over time. Almost all existing methods are replay-based with a softmax classifier. However, the inherent \textit{logits bias} problem in the softmax classifier is a main cause of catastrophic forgetting while existing solutions are not applicable for online settings. To bypass this problem, we abandon the softmax classifier and propose a novel generative framework based on the feature space. In our framework, a generative classifier which utilizes replay memory is used for inference, and the training objective is a pair-based metric learning loss which is proven theoretically to optimize the feature space in a generative way. In order to improve the ability to learn new data, we further propose a hybrid of generative and discriminative loss to train the model. Extensive experiments on several benchmarks, including newly introduced task-free datasets, show that our method beats a series of state-of-the-art replay-based methods with discriminative classifiers, and reduces catastrophic forgetting consistently with a remarkable margin.
\end{abstract}

\section{Introduction}\label{sec1}
%CL
Humans excel at continually learning new skills and accumulating knowledge throughout their lifespan. However, when learning a sequential of tasks emerging over time, neural networks notoriously suffer from \textit{catastrophic forgetting}~\cite{1989cataf} on old knowledge. This problem results from non-i.i.d distribution of data streams in such a scenario. To this end, \textit{continual learning} (CL)~\cite{parisireview,langereview} has been proposed to bridge the above gap between intelligent agents and humans.%14r, which has become a challenging but important machine learning problem.
%多了一行
%OCL

In common CL settings, there are clear boundaries between distinct tasks which are known during training. Within each task, a batch of data are accumulated and the model can be trained offline with the i.i.d data. Recently, online CL~\cite{gss,mir} setting has received growing attention in which the model needs to learn from a non-i.i.d data stream in online settings. At each iteration, new data are fed into the model only once and then discarded. In this manner, task boundary is not informed, and thus online CL is compatible with task-free~\cite{task-free,dpm} scenario. In real-world scenarios, the distribution of data stream changes over time gradually instead of switching between tasks suddenly. Moreover, the model is expected to quickly adapt to large amount of new data, e.g. user-generated content. Online CL meets these requirements, so it is more meaningful for practical applications. Many existing CL works deal with task-incremental learning (TIL) setting~\cite{ewc,lwf}, in which task identity is informed during test and the model only needs to classify within a particular task. However, for online CL problem, TIL is not realistic because of the dependence on task boundary as discussed above and reduces the difficulty of online CL. In contrast, \textit{class-incremental learning} (CIL) setting~\cite{icarl} requires the model to learn new classes continually over time and classify samples over all seen classes during test. Thus, \textit{online CIL} setting is more suitable for online data streams in real-world CL scenarios~\cite{aser}.


%, but also is not compatible with task-free scenario, where the concept of task does not exist at all. 


%CIL is challenging and such a setting is more suitable for online data stream in real-world scenarios. 

%Many CL works deal with \textit{task-incremental learning} (TIL) setting~\cite{ewc,lwf}. In this setting, the model possesses one separate output layer for each task. During test task identity is available and the model only needs to classify within a particular task. This setting not only weakens the difficulty of practical CL scenarios, but also is not compatible with task-free scenario, where the concept of task does not exist at all. 

%existing methods and motivation
Most existing online CIL methods are based on experience replay (ER)~\cite{er,mer} strategy which stores a subset of learned data in a replay memory and uses the data in memory to retrain model thus alleviating forgetting. Recently, in CIL setting \textit{logits bias} problem in the last fully connected (FC) layer, i.e. softmax classifier, is revealed~\cite{bic}, which is a main cause of catastrophic forgetting. In Figure \ref{fig1:a}, we show in online CIL, even if ER is used, logits bias towards newly learned classes in the softamx classifier is still serious and the forgetting on old tasks is dramatic (See Figure \ref{fig1:b}). Although some works~\cite{bic,il2m,wa} propose different methods to reduce logits bias, they all depend on task boundaries and extra offline phases during training so that not applicable for online CIL setting.

\begin{figure}[tb]
%\setlength{\abovecaptionskip}{0.1cm}
%\setlength{\belowcaptionskip}{-0.3cm}
\centering
\subfloat[]{\label{fig1:a} \includegraphics[height=0.17\textwidth]{fig1b.pdf}}
\subfloat[]{\label{fig1:b} \includegraphics[height=0.17\textwidth]{fig1a.pdf}}
\caption{Logits bias phenomenon of softmax classifier (left) and accuracy \& forgetting on different tasks using softmax vs. generative NCM classifier (right). The results are obtained with ER and 1k replay memory on 5-task Split CIFAR10.}
\label{fig1}
\end{figure}

In this paper, we propose to tackle the online CIL problem without the softmax classifier to avoid logits bias problem. Instead, we propose a new framework where training and inference are both in a generative way. We are motivated by the insight that generative classifier is more effective in low data regime than discriminative classifier which is demonstrated by \cite{ng01}. Although the conclusion is drawn on simple linear models~\cite{ng01}, similar results are also observed on deep neural networks (DNNs)~\cite{textgen,nligen} recently. It should be noticed that in online CIL setting the data is seen only once, not fully trained, so it is analogous to the low data regime in which the generative classifier is preferable. In contrast, the commonly used softmax classifier is a discriminative model. 

Concretely, we abandon the softmax FC layer and introduce \textit{nearest-class-mean} (NCM) classifier~\cite{ncm} for inference, which can be interpreted as classifying in a generative way. The NCM classifier is built on the feature space on the top of previous network layers. Thanks to ER strategy, NCM classifier can utilize the replay memory for inference. As for training, inspired by a recent work~\cite{unifymi}, which shows pair-based deep metric learning (DML) losses can be interpreted as optimizing the feature space from a generative perspective, we introduce Multi-Similarity (MS) loss~\cite{ms} to obtain a good feature space for NCM classifier. Meanwhile, we prove theoretically that MS loss is an alternative to a training objective of the generative classifier. In this way, we can bypass logits bias. 

%meanwhile the newly introduced NCM classifier is non-parametric which is less prone to suffer from catastrophic forgetting. %To train the generative classifier, we firstly resort to 

%the connection between this type of loss and generative models 
%with standard Gaussian distribution. 
To strengthen the model's capable of learning from new data in complex data streams, we further introduce an auxiliary proxy-based DML loss~\cite{pnca}. Therefore, our whole training objective is a hybrid of generative and discriminative losses. During inference, we ignore the discriminative objective and classify with the generative NCM classifier. By tuning weight of the auxiliary loss, our method can work well in different data streams.

In summary, our \textit{contributions} are as follows:
\begin{enumerate}
\item We make the first attempt to avoid logits bias problem in online CIL setting. In our generative framework, a generative classifier is introduced to replace softmax classifier for inference and for training, we introduce MS loss which is proven theoretically to optimize the model in a generative way.
\item In order to improve the ability of MS loss to learn from new data, we further introduce an auxiliary loss to achieve a good balance between retaining old knowledge and learning new knowledge. %By tuning the weight of the auxiliary loss, our method can work well in different data streams.
\item We conduct extensive experiments on four benchmarks in multiple online CIL settings, including a new task-free setting we design for simulating more realistic scenarios. Empirical results demonstrate our method outperforms a variety of state-of-the-art replay-based methods substantially, especially alleviating catastrophic forgetting significantly. 
\end{enumerate}

\section{Related Work}\label{sec2}
Current CL methods can be roughly divided into three categories: which are regularization, parameter isolation and replay-based respectively~\cite{langereview}. \textit{Regularization} methods retain the learned knowledge by imposing penalty constraints on model's parameters~\cite{ewc} or outputs~\cite{lwf} when learning new data. They work well in TIL setting but poor in CIL setting~\cite{3sc}. \textit{Parameter isolation} methods assign a specific subset of model parameters, such as network weights~\cite{packnet} and sub-networks~\cite{pathnet} to each task to avoid knowledge interference and thus the network may keep growing. This type of method is mainly designed for TIL as task identity is usually necessary during test. The mainstream of \textit{Replay-based} methods is ER-like~\cite{icarl}, which stores a subset of old data and retrains it when learning new data to prevent forgetting of old knowledge. In addition, generative replay method trains a generator to replay old data approximately~\cite{dgr}.

In the field of online CL, most of methods are on the basis of ER. \cite{tiny} first explored ER in online CL settings with different memory update strategies. Authors suggested ER method should be regarded as an important baseline as in this setting it is more effective than several existing CL methods, such as A-GEM~\cite{agem}. GSS~\cite{gss} designs a new memory update strategy by encouraging the divergence of gradients of samples in memory. MIR~\cite{mir} is proposed to select the maximally interfered samples from memory for replay. GMED~\cite{gmed} edits the replay samples with gradient information to obtain samples likely to be forgotten, which can benefit the replay in the future. \cite{aser} focus on online CIL setting and adopt the notion of Shapley Value to improve the replay memory update and sampling. All of the above methods are replay-based with softmax classifier. A contemporary work \cite{cpe} proposes CoPE,  which is somewhat similar to our method. CoPE replaces softmax classifier with a prototype-based classifier which is non-parametric and updated using features of data samples. However, the loss function of CoPE is still discriminative and the way to classify is analogous to softmax classifier.

Apart from the above ER based methods, \cite{bgd} propose an online regularization method, however it performs very badly in online CL settings \cite{gmed}. \cite{dpm} propose a parameter isolation method in which the network is dynamically expanded and a memory for storing data is still required. Therefore, the memory usage is not fixed and potentially unbounded.

A recent work~\cite{sdc} proposes SDC, a CIL method based on DML and NCM classifier. However, SDC requires an extra phase to correct semantic drift  after training each task. This phase depends on task boundaries and the accumulated data of a task, which is not applicable for online CIL. In contrast, our method is based on ER and classifies with replay memory and thus need not correct the drift. 
\section{Online Class-Incremental Learning with a Generative Framework}
\subsection{Preliminaries and Motivations}
\subsubsection{Online Class-Incremental Learning} CIL setting has been widely used in online CL literature, e.g.~\cite{mir,aser}, and a softmax classifier is commonly used. A neural network $f(\cdot;\tt):\mathcal{X}\to\mathbb{R}^d$ parameterized by $\tt$ encodes data samples $\x\in\mathcal{X}$ into a $d$-dimension feature $f(\x)$ on which an FC layer $g$ outputs logits for classification: $\logit=\mathbf{W}f(\x)+\mathbf{b}$. At each iteration, a minibatch of data $\newbatch$ from a data stream $\mathcal{S}$ arrives and the whole model $(f,g)$ is trained on $\newbatch$ only once. The training objective is cross-entropy (CE) loss:
\begin{equation}\label{eq1}
\mathcal{L}_{CE}=-\sum_{c=1}^{\tilde{C}} \t_{:c}\log\haty_{:c}, \quad \haty_{:c}=\frac{e^{\logit_{:c}}}{\sum_{c=1}^{\tilde{C}} e^{\logit_{:c}}}
\end{equation}

\noindent where $\tilde{C}$ is the number of classes seen so far. $\t$ is one-hot label of $\x$ and the subscript $:\!c$ denotes the $c$-th component. The new classes from $\mathcal{S}$ emerge over time. The output space of $g$ is the number of seen classes and thus keeps growing. At test time, the model should classify over all $C$ classes seen. %A common setting is there are clear task boundaries in $\mathcal{S}$ and each task has the same number of classes. However, in more general task-free setting, the new classes emerge irregularly. 
\subsubsection{Experience Replay for Online Continual Learning}
ER makes two modifications during online training: (1) It maintains a replay memory $\memory$ with limited size which stores a subset of previously learned samples. (2) When a minibatch of new data $\newbatch$ is coming, it samples a minibatch $\replaybatch$ from $\memory$ and uses $\newbatch \cup \replaybatch$ to optimize the model with one SGD-like step. Then it updates $\memory$ with $\newbatch$. Recent works, e.g.~\cite{mir,aser} regard ER-reservoir as a strong baseline, which combines ER with reservoir sampling~\cite{reservoir} for memory update and random sampling for $\replaybatch$. See \cite{tiny} for more details about it.
\subsubsection{Logits Bias in Softmax Classifier}
Some recent works~\cite{bic,il2m,wa} show in CIL scenarios, even with replay-based mechanism the logits outputted by model always have a strong bias towards the newly learned classes, which leads to catastrophic forgetting actually. In preliminary experiments, we also observe this phenomenon in online CIL setting. We run ER-reservoir baseline on 5-task Split CIFAR10 (each task has two disjoint classes) online CIL benchmark. In Figure \ref{fig1:a}, we display the average logits of each already learned tasks over samples in test data after learning each task. The model outputs much higher logits on the new classes (of the task just learned) than old classes. 

Following \cite{gradient}, we examine the % softmax classifier and 
CE loss in Eq~(\ref{eq1}), the gradient of $\mathcal{L}_{CE}$ w.r.t logit $\logit_{:c}$ of class $c$ is $\haty_{:c}-\mathbb{I}[\t_{:c}=1]$.
%as follows: \partial\mathcal{L}_{CE}/\partial \logit_{c}=
%\begin{equation}\label{eq2}
%\partial\mathcal{L}_{CE}/\partial \logit_{c}=\haty_{c}-\mathbb{I}[\t_{c}=1]
%\end{equation}
Thus, if $c$ is the real label $y$, i.e. $\t_{:c}=1$, the gradient is non-positive and model is trained to increase $\logit_{:c}$, otherwise the gradient is non-negative and model is trained to decrease $\logit_{:c}$. Therefore, \textit{logits bias} problem is caused by the imbalance between the number of samples of the new classes and that of the old classes with a limited size of $\memory$. 
%$\frac{\partial \mathcal{L}_{CE}}{\partial \logit_{c}}\leq 0$, and model is trained to increase $\logit_{c}$. Otherwise $\frac{\partial \mathcal{L}_{CE}}{\partial \logit_{c}}\geq 0$, and model decreases $\logit_{c}$.
%Therefore, in online CIL setting, \textit{logits bias} is caused by the imbalance between the number of old class samples in $\replaybatch$ and new class samples in $\newbatch$ as the size of $\replaybatch$ is always limited to be equal to $\newbatch$. Most of the time the model is optimized to increase new classes's logits and reduce old classes's logits. 
As mentioned in Section~\ref{sec1}, existing solutions~\cite{bic,il2m,wa} designed for conventional CIL need task boundaries to conduct extra offline training phases and even depend on the accumulated data of one task. They are not applicable for online CIL setting where task boundaries are not informed or even do not exist in task-free scenario.
%where the data samples come from the streams and is discarded after training once. Especially, for task-free scenarios, the task boundary does not exist thus the model cannot be aware when these solutions should be conducted.

\subsection{Inference with a Generative Classifier}\label{ncm}
Proposed generative framework is based on ER strategy, and aims to avoid the intrinsic logits bias problem by removing the softmax FC layer $g$ and build a generative classifier on the feature space $\mathcal{Z}: \z=f(\x)$. If the feature $\z$ is well discriminative, we can conduct inference with samples in $\memory$ instead of a parametric classifier which is prone to catastrophic forgetting~\cite{icarl}. We use NCM classifier firstly suggested by~\cite{icarl} for CL and show it is a generative model. We use $\memory_c$ to denote the subset of class $c$ of $\memory$. The class mean $\bmu_c$ is computed by $\bmu_c^{\memory}=\frac{1}{|\mathcal{M}_c|}\sum_{\x\in\mathcal{M}_c}f(\x)$.
During inference, the prediction for $\x^*$ is made by: 
\begin{equation}\label{eq3}
y^{*}=\mathop{\arg\min}_{c} \|f(\x^*)-\bmu_c^{\memory} \|_2
\end{equation}

In fact, the principle of prediction in Eq~(\ref{eq3}) is to find a Gaussian distribution $\mathcal{N}(f(\x^*)|\bmu_c^{\memory},\mathbf{I})$ with the maximal probability for $\x^*$. Therefore, assuming the conditional distribution $p(\z|y=c)=\mathcal{N}(\z|\bmu_c^{\memory},\mathbf{I})$ and the prior distribution $p(y)$ is uniform, NCM classifier virtually deals with $p(y|\z)$ by modeling $p(\z|y)$ in a generative way. The inference way is according to Bayes rule: $\mathop{\arg\max}p(y|\x^*)=\mathop{\arg\max}p(f(\x^*)|y)p(y)$. The assumption about $p(y)$ simplifies the analysis and works well in practice. In contrast, softmax classifier models $p(y|\x^*)$ in a typical discriminative way.

%On simple linear models, \cite{ng01} demonstrate that although discriminative classifiers have lower asymptotic error than generative classifier, the latter is more effective in low data regime. Some recent works also show generative classifiers are preferable in low data regime on DNNs~\cite{textgen,nligen}. 
As discussed above, online CIL is in a low data setting where generative classifiers are preferable compared to discriminative classifiers~\cite{ng01}. Moreover, generative classifiers are more robust to continual learning~\cite{textgen} and imbalanced data settings~\cite{nligen}. At each iteration, $\newbatch \cup \replaybatch$ is also highly imbalanced. Considering these results, we hypothesis generative classifiers are promising for online CIL problem. It should be noted our method only models a simple generative classifier $p(\z|y)$ on the feature space, instead of modeling $p(\x|y)$ on the input space using DNNs~\cite{textgen}, which is time-consuming and thus is not suitable for online training. 
%\subsection{Training Generative Classifier with a Pair-based Metric Learning Loss}

%以上可以再加一行
\subsection{Training with a Pair-based Metric Learning Loss from a Generative Perpective}
To train the feature extractor $f(\tt)$ we resort to DML losses which aim to learn a feature space where the distances represent semantic dissimilarities between data samples. From the perspective of mutual information (MI), \cite{unifymi} theoretically show the equivalence between CE loss and several pair-based DML losses, such as contrast loss~\cite{constrast} and Multi-Similarity (MS) loss~\cite{ms}. The DML losses maximize MI between feature $\z$ and label $y$ in a generative way while CE loss in a discriminative way, which motivates us to train $f(\tt)$ with a pair-based DML loss to obtain a good feature space $\mathcal{Z}$ for the generative classifier. 

Especially, we choose the MS loss as a training objective. MS loss is one of the state-of-the-art methods in the field of DML. \cite{ms} point out pair-based DML losses can be seen as weighting each feature pair in the general pair weighting framework. As MS loss requires the feature $f(\x)$ to be $\ell_2$-normalized first, from now on, we use $\z_i$ to denote the $\ell_2$-normalized feature of $\x_i$ and a feature pair is represented in the form of inner product $\Scos_{ij}\coloneqq\z_i^{\mathrm{T}}\z_j$. To weight feature pairs better, MS loss is proposed to consider multiple types of similarity. MS loss on a dataset $\mathcal{D}$ is formulated as follows:

\begin{equation}    
\begin{aligned}
 \mathcal{L}_{MS}(\mathcal{D})=&\frac{1}{|\mathcal{D}|}\sum_{i=1}^{|\mathcal{D}|}\big\{\frac{1}{\alpha}\log [1+\sum_{j\in\mathcal{P}_i}e^{-\alpha(\Scos_{ij}-\lambda)}]\\
 &+\frac{1}{\beta}\log [1+\sum_{j\in\mathcal{N}_i}e^{\beta(\Scos_{ij}-\lambda)}] \big\}     
\end{aligned}
\end{equation}  

where $\alpha$, $\beta$ and $\lambda$ are hyperparameters and $\mathcal{P}_i$ and $\mathcal{N}_i$ represent the index set of positive and negative samples of $\x_i$\footnote{The positive samples have the same labels as $\x_i$ while the negative samples have different labels from $\x_i$.} respectively. MS loss also utilizes the hard mining strategy to filter out too uninformative feature pairs, i.e. too similar positive pairs and too dissimilar negative pairs:
\begin{equation}\label{hm}
\begin{split}
    \mathcal{P}_i=\{j|\Scos_{ij}<\mathop{\max}_{y_k\neq y_i}\Scos_{ik}+\epsilon\} \quad  \mathcal{N}_i=\{j|\Scos_{ij}>\mathop{\min}_{y_k=y_i}\Scos_{ik}-\epsilon\}
\end{split}
\end{equation}
where $\epsilon$ is another hyperparameter in MS loss. At each iteration we use MS loss on the union of new samples and replay samples $\mathcal{L}_{MS}(\newbatch \cup \replaybatch)$ to train the model. The sampling of $\replaybatch$ and update of $\memory$ are the same as ER-reservoir.

To show the connection between $\mathcal{L}_{MS}$ and the generative classifier in Eq~(\ref{eq3}), we conduct some theoretical analyses. 

\begin{proposition}\label{prop1}
Assume dataset $\mathcal{D}=\{(\x_i,y_i)\}_{i=1}^n$ is class-balanced and has $C$ classes each of which has $n_0$ samples. For a generative model $p(\z,y)$, assume $p(y)$ actually obeys the uniform distribution and $p(\z|y=c)=\mathcal{N}(\z|\bmu_c^{\mathcal{D}},\mathbf{I})$ where $\bmu_c^{\mathcal{D}}=\frac{1}{n_0}\sum_{i=1}^n\z_i\mathbb{I}[y_i=c]$. 
For MS loss assume hard mining in Eq~(\ref{hm}) is not employed. Then we have:
\begin{equation}
\mathcal{L}_{MS}\cgeq \mathcal{L}_{Gen-Bin}
\end{equation}
where $\cgeq$ stands for upper than, up to an additive constant c and $\mathcal{L}_{Gen-Bin}$ is defined in the following:
\begin{equation}\label{genbin}
\begin{aligned}
% \frac{1}{n}\sum_{i=1}^n\big\{-\log p(\zi|y_i)+\frac{1}{C-1}\sum_{c:c\neq y_i}\log p(\zi|c)\big\}
 \mathcal{L}_{Gen-Bin}=&-\frac{1}{n}\sum_{i=1}^n \log p(\zi|y=y_i) \\
 &+ \frac{1}{nC}\sum_{i=1}^n \sum_{c=1}^C\log p(\zi|y=c)
 \end{aligned}
\end{equation}
\end{proposition}
The proof of Proposition \ref{prop1} is in Appendix. Proposition \ref{prop1} shows $\mathcal{L}_{MS}$ is an upper bound of $\mathcal{L}_{Gen-Bin}$ and thus is an alternative to minimizing $\mathcal{L}_{Gen-Bin}$. The first term of $\mathcal{L}_{Gen-Bin}$ aims to minimize the negative log-likelihood of the class-conditional generative classifier, while the second term maximizes the conditional entropy $H(Z|Y)$ of labels $Y$ and features $Z$. It should be noticed $\mathcal{L}_{Gen-Bin}$ depends on modeling $p(\z|y)$. With uniform $p(y)$, classifying using $p(\z|y)$ equals to classifying using $p(\z,y)$, and $H(Z|Y)$ is equivalent to $H(Z, Y)$, which can be regarded as a regularizer against features collapsing. Thus, $\mathcal{L}_{Gen-Bin}$ actually optimizes the model in a generative way. The assumptions in Proposition \ref{prop1} are similar with those in Section \ref{ncm} about NCM classifier. The difference lies in that NCM classifier uses $\{\bmu_c^{\memory}\}$ computed on replay memory $\memory$ to approximate $\{\bmu_c^{\D}\}$. Therefore, Proposition \ref{prop1} reveals that MS loss optimizes the feature space in a generative way and it models $p(\z|y)$ for classification which is consistent with the NCM classifier.

The real class means $\{\bmu_c^{\D}\}$ depend on all training data and change with the update of $f(\tt)$ so that are intractable in online settings. MS loss can be efficiently computed as it does not depend on $\{\bmu_c^{\D}\}$ thus the model can be trained efficiently. During inference, we use approximate class means $\bmu_c^{\memory}$ to classify. In Figure~\ref{fig1:b}, on 5-task Split CIFAR10 benchmark, we empirically show compared to softmax classifier, on old tasks, our method achieves much higher accuracy and much lower forgetting, which implies MS loss is an effective objective to train the model $f$ and class mean $\bmu_c^{\memory}$ of replay memory is a good approximation of $\bmu_c^{\D}$. 


With discriminative loss like CE loss, the classifier models a discriminative model $p(y|\z)$. Therefore, if training with discriminative loss and inference with NCM classifier based on the generative model $p(\z|y)$, we can not expect to obtain good results. In the next section, experiments will verify this conjecture. In contrast, the way to train and inference are coincided in proposed generative framework. 

%We will show empirically $\bmu$ works  

\begin{table*}[htb]
%\setlength{\abovecaptionskip}{0.1cm}
%\setlength{\belowcaptionskip}{-0.2cm}
\small
\begin{center}
\scalebox{0.9}{
\begin{tabular}{c|cccccc}
\toprule[1.0pt]
Methods &\tabincell{c}{MNIST\\(5-task)} &\tabincell{c}{CIFAR10 \\(5-task)} &\tabincell{c}{CIFAR100 \\(10-task)} &\tabincell{c}{CIFAR100 \\(20-task)}&\tabincell{c}{miniImageNet \\(10-task)}&\tabincell{c}{miniImageNet \\(20-task)}\\  \hline \hline \specialrule{0em}{1.0pt}{1.0pt}
fine-tune &19.66$\pm$0.05 &18.40$\pm$0.17& 6.26$\pm$0.30 &3.61$\pm$0.24 &4.43$\pm$0.19&3.12$\pm$0.15\\
ER-reservoir &82.34$\pm$2.48 &39.88$\pm$1.52& 11.59$\pm$0.26&8.95$\pm$0.26&10.24$\pm$0.41 &8.33$\pm$0.66\\
A-GEM
&25.99$\pm$1.62 &18.01$\pm$0.17
&6.48$\pm$0.18 &3.66$\pm$0.09
&4.68$\pm$0.11 &3.37$\pm$0.13 \\
GSS-Greedy&83.88$\pm$0.72 &39.07$\pm$2.02&
10.78$\pm$0.28&7.94$\pm$0.47&9.20$\pm$0.61&7.76$\pm$0.35\\
MIR&86.81$\pm$0.95 &42.10$\pm$1.27&11.52$\pm$0.37&8.61$\pm$0.34&9.99$\pm$0.49&7.93$\pm$0.70\\ 
GMED-ER
& 81.71$\pm$1.87&42.65$\pm$1.27
& 11.86$\pm$0.36&9.16$\pm$0.47
& 9.53$\pm$0.66&8.14$\pm$0.58\\
GMED-MIR
& 88.70$\pm$0.81&44.53$\pm$2.23
& 11.58$\pm$0.51&8.48$\pm$0.37
& 9.24$\pm$0.53&7.75$\pm$0.80
\\
CoPE
& 87.58$\pm$0.65&47.36$\pm$0.96
& 10.79$\pm$0.36&9.11$\pm$0.44
& 11.03$\pm$0.68&9.92$\pm$0.61\\
ASER$_{\mu}$ $^\ast$ &-- &43.50$\pm$1.40& 14.00$\pm$0.40&--& 12.20$\pm$0.80& --\\
\specialrule{0em}{0.5pt}{0.5pt} \hline \specialrule{0em}{0.5pt}{0.5pt}
Ours
&\textbf{88.79$\pm$0.26}
&\textbf{51.84$\pm$0.91} 
&\textbf{15.56$\pm$0.39}
&\textbf{13.65$\pm$0.35}
&\textbf{16.05$\pm$0.38}
&\textbf{15.15$\pm$0.36}\\  \hline \specialrule{0em}{0.5pt}{0.5pt}
i.i.d. online  &86.35$\pm$0.64&62.37$\pm$1.36 &20.62$\pm$0.48& 20.62$\pm$0.48 &18.02$\pm$0.63&18.02$\pm$0.63\\
i.i.d. offline  &92.44$\pm$0.61 &79.90$\pm$0.51&45.59$\pm$0.29& 45.59$\pm$0.29&38.63$\pm$0.59&38.63$\pm$0.59 \\ \hline
\bottomrule[1.0pt] 
\end{tabular}
}
\end{center}
\caption{Average Accuracy of 15 runs on \textit{Split} datasets. Higher is better. $^\ast$ indicates the results are from the original paper.}
\label{table1}
\end{table*}
\subsection{A Hybrid Generative/Discriminative Loss}
However, when addressing classification tasks, generative classifier has natural weakness, since modeling joint distribution $p(\x, y)$ is much tougher than modeling conditional distribution $p(y|\x)$ for NNs. Moreover, in preliminary experiments, we found if only trained with MS loss, the NCM classifier's performance degenerates as the expected number of classes in $\newbatch$ at each iteration increases. This phenomenon is attributed to the inadequate ability to learn from new data, instead of catastrophic forgetting. We speculate because the size of $\newbatch$ is always fixed to a small value (e.g. 10) in online CIL settings, the number of positive pairs in $\newbatch$ decreases as the expected number of classes increases. 

To remedy this problem, we take advantage of discriminative losses for fast adaptation in online setting. To this end, we introduce Proxy-NCA (PNCA)~\cite{pnca}, a proxy-based DML loss, as an auxiliary loss. For each class, PNCA loss maintains ``proxies'' as the real feature to utilize the limited data in a minibatch better, which leads to convergence speed-up compared to pair-based DML losses. Concretely, when a new class $c$ emerges, we assign one trainable proxy $\p_c\in \mathbb{R}^d$ to it. %Let $\tilde{C}$ denote the number of already seen classes. 
PNCA loss is computed as:
\begin{equation}
\mathcal{L}_{PNCA}(\D)=-\frac{1}{|\D|}\sum_{(x,y)\in \D}\log\frac{e^{-\|f(\x)-\p_y\|_2^2}}{\sum_{c=1}^{\tilde{C}}e^{-\|f(\x)-\p_c\|_2^2}}
\end{equation}
\cite{pnca} suggest all proxies have the same norm $N_P$ and all features have the norm $N_F$. The latter satisfies as in MS loss the feature is $\ell_2$-normalized, i.e. $N_F=1$. We also set $N_P=1$ by normalizing all proxies after each SGD-like update. In this way, $\mathcal{L}_{PNCA}$ is equivalent to a CE loss with $\ell_2$-normalized row vectors of $\mathbf{W}$ and without bias $\mathbf{b}$, and thus we use PNCA instead of CE loss to keep utilizing the normalized features of MS loss. Our full training objective is a hybrid of generative and discriminative losses:
\begin{equation}\label{hybrid}
\mathcal{L}_{Hybrid}=\mathcal{L}_{MS}+\gamma\mathcal{L}_{PNCA}
\end{equation}  
where $\gamma$ is a hyperparameter to control the weight of $\mathcal{L}_{PNCA}$. In general, generative classifiers have a smaller variance but higher bias than discriminative classifiers, and using such a hybrid loss can achieve a better bias-variance tradeoff~\cite{hybrid04}. Thus we think introducing the discriminative loss $\mathcal{L}_{PNCA}$ can reduce the bias of model so that boost the ability to learn from new data.

It should be noticed we train the model with $\mathcal{L}_{Hybrid}(\newbatch\cup \replaybatch)$, while we only use NCM classifier in Eq~(\ref{eq3}) for inference. In all experiments, we set $\alpha=2$, $\beta=50$, $\epsilon=0.1$ following~\cite{ms} and $\lambda=0.5$ which always works well in online CIL settings. We only need to tune hyperparemeters $\gamma$ in Eq~(\ref{hybrid}) for different experiment settings.

\section{Experiments}
\subsection{Experiment Setup}
\begin{table*}[h]
%\setlength{\abovecaptionskip}{0.1cm}
%\setlength{\belowcaptionskip}{-0.2cm}
\small
\begin{center}
\scalebox{0.9}{
\begin{tabular}{c|cccccc}
\toprule[1.0pt]
Methods &\tabincell{c}{MNIST\\(5-task)} &\tabincell{c}{CIFAR10 \\(5-task)} &\tabincell{c}{CIFAR100 \\(10-task)} &\tabincell{c}{CIFAR100 \\(20-task)}&\tabincell{c}{miniImageNet \\(10-task)}&\tabincell{c}{miniImageNet \\(20-task)}\\ \hline \hline \specialrule{0em}{1.0pt}{1.0pt}
fine-tune &99.24$\pm$0.09 &85.45$\pm$0.63& 51.60$\pm$0.77 &65.51$\pm$0.78 &41.12$\pm$0.82&52.99$\pm$0.89\\
ER-reservoir
&18.33$\pm$1.77 &52.72$\pm$1.90
&45.94$\pm$0.55 &57.31$\pm$0.71
&36.05$\pm$0.78 &47.70$\pm$0.90\\
A-GEM 
&89.90$\pm$2.02 &82.80$\pm$0.73
&54.15$\pm$0.42 &67.61$\pm$0.53
&43.31$\pm$0.52 &54.47$\pm$0.78
\\
GSS-Greedy
&15.13$\pm$0.99&49.96$\pm$2.82
&44.30$\pm$0.57&53.87$\pm$0.54
&36.17$\pm$0.58&45.91$\pm$0.79
\\
MIR
&9.71$\pm$1.39&44.34$\pm$2.65
&46.52$\pm$0.52&56.58$\pm$0.62
&36.98$\pm$0.78&45.84$\pm$1.11\\
GMED-ER
& 16.21$\pm$2.70&44.93$\pm$1.68
& 46.35$\pm$0.50&57.76$\pm$0.94
& 35.22$\pm$1.16&45.08$\pm$1.28
\\
GMED-MIR
& 12.52$\pm$1.05&39.88$\pm$2.23
& 46.56$\pm$0.65&58.14$\pm$0.55
& 34.79$\pm$1.01&45.50$\pm$1.49
\\
CoPE
& 9.51$\pm$1.15&40.01$\pm$1.80
& 36.51$\pm$0.86&43.82$\pm$0.62
& 29.43$\pm$0.98&40.99$\pm$1.02

\\
ASER$_{\mu}$ $^\ast$ 
&-- &47.90$\pm$1.60
&45.00$\pm$0.70&--
&28.00$\pm$1.30&--\\
\specialrule{0em}{0.5pt}{0.5pt} \hline \specialrule{0em}{0.5pt}{0.5pt}
Ours
&9.36$\pm$0.37&\textbf{35.37$\pm$1.35} &\textbf{21.79$\pm$0.69}&\textbf{27.10$\pm$1.10}
&\textbf{21.26$\pm$0.59}&\textbf{24.98$\pm$0.87}\\ \hline \specialrule{0em}{0.5pt}{0.5pt}
\bottomrule[1.0pt] 
\end{tabular}
}
\end{center}

\caption{Average Forgetting of 15 runs on \textit{Split} datasets. Lower is better. $^\ast$ indicates the results are from the original paper.}
\label{table2}
\end{table*}
\begin{figure}[tb]
\centering
\includegraphics[height=0.15\textwidth]{figs1.pdf}
\caption{The probability distribution on class of the sample at each time step on Split CIFAR10 (left) and Smooth CIFAR10 (right).}
\label{figs1}

\end{figure}


\textbf{Datasets} First, we conduct experiments on \textit{Split} datasets which are commonly used in CIL and online CIL literature. On Split MNIST and CIFAR10, the datasets are split into 5 tasks each of which comprises 2 classes. On CIFAR100 and miniImageNet with 100 classes, we split them into 10 or 20 tasks. The number of classes in each task is 10 or 5 respectively. For MNIST we select 5k samples for training following~\cite{mir} and we use full training data for other datasets. To simulate a task-free scenario, task boundaries are not informed during training~\cite{gmed}. 

To conduct a thorough evaluation in task-free scenarios, we design a new type of data streams. For a data stream with $C$ classes, we assume the length of stream is $n$ and $n_0=n/C$. We denote $p_c(t)$ as the occurrence probability of class $c$ at time step $t$ and assume $p_c(t) \sim\mathcal{N}(t|(2c-1)n_0/2,n_0/2)$. At each time step $t$, we calculate ${\bm p}(t)=(p_1(t),\dots,p_C(t))$ and normalize ${\bm p}(t)$ as the parameters of a Categorical distribution from which a class index $c_t$ is sampled. Then we sample one data of class $c_t$ without replacement. In this setting, data distribution changes smoothly and there is no notion of task. We call such data streams as \textit{Smooth} datasets. To build Smooth datasets, we set $n=5k$ on CIFAR10 and $n=40k$ on CIFAR100 and miniImageNet, using all classes in each dataset. For all datasets, the size of minibatch $\newbatch$ is 10. In Figure~\ref{figs1} we plot the probability distribution on class at each time step in the data stream generation process for Split CIFAR10 and Smooth CIFAR10. For better comparison, we set the length of data stream of two datasets both 5k. Split CIFAR10 has clear task boundaries and within one task the distribution on class is unchanged and uniform. However, On Smooth CIFAR10, the distribution on class keeps changing and there is no notion of task. 
\begin{figure}[tb]
\centering

\includegraphics[height=0.18\textwidth]{fig2.pdf}
\caption{Average Accuracy on already learned task during training.}
\label{fig2}
\end{figure}

\textbf{Baselines} We compare our method against a series of state-of-the-art online CIL methods, including: ER-reservoir, A-GEM, GSS, MIR, GMED, CoPE and ASER. We have briefly introduced them in Section~\ref{sec2}. Specially, we use GSS-greedy and ASER$_{\mu}$ which are the best variants in the corresponding paper. For GMED, we evaluate both GMED-ER and GMED-MIR. We also evaluate fine-tune baseline without any CL strategy. For all baselines and our method, the model is trained with 1 epoch, i.e. online CL setting. In addition, the performances of i.i.d online and i.i.d offline are also provided, by training the model 1 and 5 epochs respectively on i.i.d data streams. We reimplement all baselines except ASER$_{\mu}$, whose results are from the original paper.

\textbf{Model} Following~\cite{mir}, the model $f$ is a 2-layer MLP with 400 hidden units for MNIST and a reduced ResNet18 for other datasets. For baselines with ER strategy, the size of replay minibatch $\replaybatch$ is always 10. The budget of memory $\memory$ is 500 on MNIST and 1000 on others. We use a relatively small budget $|\memory|$ to mimic a practical setting. All models are optimized by SGD. The \textit{single-head evaluation} is always used for CIL.
%According to validation we set $\gamma=0.1$ on MNIST and CIFAR10, $\gamma=0.5$ on CIFAR100 and $\gamma=1.0$ on miniImageNet.






\begin{figure}
\centering

    \subfloat[]{\label{fig3:a} \includegraphics[height=0.16\textwidth]{fig3a.pdf}}\hspace{0mm}
    \subfloat[]{\label{fig3:b} \includegraphics[height=0.16\textwidth]{fig3b.pdf}}
    \caption{Comparison of training time (a) and test time (b) on Split CIFAR100 and miniImageNet. The number of tasks is 10.}
    \label{fig3}
    %\end{figure}
   

   
\end{figure}
   
  \begin{table}[th]
    \centering
    \small
    \scalebox{0.9}{
    \begin{tabular}{c|c|ccc} 
    \toprule[1.0pt]
    Training&Inference&CIFAR10&CIFAR100\\
    \hline
    \specialrule{0em}{0.5pt}{0.5pt} 
    CE loss &Softmax (Dis)& 39.88$\pm$1.52&8.95$\pm$0.26\\
    CE loss &NCM (Gen)&44.46$\pm$0.95&8.96$\pm$0.38\\
    MS loss &NCM (Gen)&51.72$\pm$1.02&9.99$\pm$0.32\\
    PNCA loss &NCM (Gen) &41.91$\pm$1.78&9.31$\pm$0.58\\
    Hybrid loss &Proxy (Dis)&48.16$\pm$1.21&7.02$\pm$0.75\\
    Hybrid loss &NCM (Gen)&51.84$\pm$0.91&13.65$\pm$0.35\\
    \bottomrule[1.0pt]  
    \end{tabular}
    }
    \caption{Ablation study on Split CIFAR10 and 20-task Split CIFAR100. We show the performances of different combinations of losses and inference ways. Dis: Discriminative, Gen: Generative.}
    \label{table3}
  \end{table}
\begin{table}[th]
\centering
    \small
    %\begin{center}
    \scalebox{0.9}{
    \begin{tabular}{c|ccc} 
    \toprule[1.0pt]
    {Method}&CIFAR10&CIFAR100&miniImageNet \\
    \hline \hline \specialrule{0em}{1.0pt}{1.0pt}
    fine-tune	&10.02$\pm$0.03	&1.02$\pm$0.03	&1.02$\pm$0.04\\
    ER-reservoir &20.89$\pm$2.07&3.84$\pm$0.42	&6.85$\pm$0.70\\
    MIR &18.75$\pm$2.53&4.35$\pm$0.53&6.09$\pm$1.04\\
    GMED-MIR &18.78$\pm$2.31&3.68$\pm$0.48&7.22$\pm$0.81\\
    \specialrule{0em}{0.5pt}{0.5pt} \hline \specialrule{0em}{0.5pt}{0.5pt}
    Ours &\textbf{34.18$\pm$0.81}&\textbf{10.54$\pm$0.38}&\textbf{12.24$\pm$0.19}\\ 
    \hline \specialrule{0em}{0.5pt}{0.5pt}
    i.i.d online	&31.23$\pm$2.11	&18.08$\pm$0.62	&17.23$\pm$0.42 \\
    i.i.d offline	&48.37$\pm$1.23	&42.68$\pm$0.37	&39.82$\pm$0.46 \\
    \hline
    \bottomrule[1.0pt]  
    \end{tabular}
    }
    %\end{center}
    \caption{Final accuracy of 15 runs on \textit{Smooth} datasets.}
    \label{table4}
    %\end{table}
\end{table}

\subsection{Main Results on \textit{Split} Datasets}
%\noindent \textbf{Accuracy and Forgetting}\indent 
On \textit{Split} datasets, we use \textbf{Average Accuracy} and \textbf{Average Forgetting} after training all tasks~\cite{tiny} for evaluation, which are reported in Table~\ref{table1} and Table~\ref{table2} respectively. For each metric, we report the mean of 15 runs and the 95\% confidence interval.
%and standard error of the mean (SEM) of 15 runs and SEM represents the 95\% confidence interval.

In Table~\ref{table1}, we can find our method outperforms all baselines on all 6 settings. The improvement of our method is significant except on MNIST, where GMED-MIR is competitive with our method. An interesting phenomenon is all existing methods do not have a substantial improvement over ER-reservoir on CIFAR100 and miniImageNet, except ASER. We argue for online CIL problem, we should pay more attention to complex settings.  Nevertheless, our method is superior to ASER obviously, especially on CIFAR10 and miniImageNet. Table~\ref{table2} shows the forgetting of our method is far lower than other methods based on the softmax classifier, except on MNIST. Figure~\ref{fig2} shows our method is almost consistently better than all baselines during the whole learning processes. 

\textbf{Ablation Study} We also conduct ablation study about training objective and classifier in Table~\ref{table3}. The ER-reservoir corresponds to the first row and our method corresponds to the last row. Firstly, we find for ER-reservoir, replacing softmax classifier with NCM classifier makes a substantial improvement on CIFAR10. However, it has no effect on more complex CIFAR100 (row 1\&2). Secondly, only using MS loss works very well on CIFAR10 while on CIFAR100 poor ability to learn from new data limits its performance (row 3\&6). Lastly, when hybrid loss is used, the NCM classifier is much better than proxy-based classifier (row 5\&6), and MS loss is critical for NCM classifier (row 4\&6). Note that hybrid loss does not outperform MS loss much on Split-CIFAR10. This is because in Split-CIFAR10, a minibatch of new data contains a maximum of two classes, and thus the positive pairs are enough fo MS loss to learn new knowledge well. These results verify our statement in Section 3.2. 



\textbf{Time Comparison} In Figure~\ref{fig3:a}, we report the training time of different methods. The training time of our method is only a bit higher than ER-reservoir. 

Most baselines, such as GSS, MIR, and GMED, improve ER-reservoir by designing new memory update and sampling strategies which depend on extra gradient computations and thus are time-consuming. The inference costs of softmax classifier and our NCM classifier are displayed in Figure~\ref{fig3:b}. We can find the extra time of NCM to compute the class means is (about 3\%) slight, as the size of memory is limited.%With the similar purpose, ASER potentially has this shortcoming.



%Discussions about SDC and uniform prior

%We define $p(\x|\y=c)\sim\mathcal{N}(\x|\bmu_c,\mathbf{I})$, where $\bmu_{c}=\frac{1}{n_{c}} \sum_{i}\left[y_{i}=c \right] \mathbf{z}_{i}$. Assuming that classes are balanced i.e. $\forall c, n_{c}\equiv n_{0}$ and features $\z$ are $\ell_2$-normalized. $\Scos_{ij}$ represents the cosine similarity between $\z_i$ and $\z_j$.


% data, baselines and Experiment Setting
% main results (accuracy and forgetting on 6 settings)
% time of training and evaluation
% visualization of feature space(optional)
% ablation study
% accuracy on smooth settings
\subsection{Results on Task-free \textit{Smooth} Datasets}
%\textit{Split} datasets are originally designed for CIL and there are clear task boundaries and each task has the same number of classes. However, in 

%In our task-free \textit{Smooth} datasets, the new classes emerge irregularly and the distribution on class changes at each time step. 
%A common setting is there are clear task boundaries in $\mathcal{S}$ and each task has the same number of classes. 
In newly designed task-free \textit{Smooth} datasets, the new classes emerge irregularly and the distribution on class changes at each time step. In Table~\ref{table4}, we compare our method with several baselines on three \textit{smooth} datasets. The metric is final accuracy after learning the whole data stream. We can find these datasets are indeed more complex as \textit{fine-tune} can only classify correctly on the last class, which is due to the higher imbalance of data streams. For this reason, baselines such as ER-reservoir and MIR degrade obviously compared with \textit{split datsets}. However, our method performs best consistently. %The detailed characteristic of smooth datasets can be found in supplemental material.  



\section{Conclusion}
In this work, we tackle with online CIL problem from a generative perspective to bypass logits bias problem in commonly used softmax classifier. We first propose to replace softmax classifier with a generative classifier. Then we introduce MS loss for training and prove theoretically that it optimizes the feature space in a generative way. We further propose a hybrid loss to boost the model's ability to learn from new data. Experimental results show the significant and consistent superiority of our method compared to existing state-of-the-art methods.

\bibliographystyle{IEEEtran}
\bibliography{ocl}



\appendix
%\textsc{S}

\subsection{Proof of Proposition 1}
\begin{proof}
For simplicity, we ignore the coefficient $\frac{1}{n}$ both in $\mathcal{L}_{MS}$ and $\mathcal{L}_{Gen-Bin}$ in the proof.
We denote the two parts in the summation of $\mathcal{L}_{MS}$ as $\mathcal{L}_{MS}^+$ and $\mathcal{L}_{MS}^-$ respectively, i.e.:
\begin{align}
\begin{split}
\mathcal{L}_{MS}^+&=\sum_{i=1}^{n}\frac{1}{\alpha}\log [1+\sum_{j\in\mathcal{P}_i}e^{-\alpha(\Scos_{ij}-\lambda)}] \\
\mathcal{L}_{MS}^-&=\sum_{i=1}^{n}\frac{1}{\beta}\log [1+\sum_{j\in\mathcal{N}_i}e^{\beta(\Scos_{ij}-\lambda)}]
\end{split}
\end{align}
Without hard mining, for $\mathcal{L}_{MS}^+$ we have:
\begin{align}\label{eqs1}
\begin{split}
\mathcal{L}_{MS}^+ &= \sum_{i=1}^{n}\frac{1}{\alpha}\log [1+\sum_{j:y_j=y_i}e^{-\alpha(\Scos_{ij}-\lambda)}] \\
&\geq \sum_{i=1}^{n}\frac{1}{\alpha}\log [\sum_{j:y_j=y_i}e^{-\alpha(\Scos_{ij}-\lambda)}]  \\
&\cgeq \sum_{i=1}^{n}\frac{1}{\alpha}[\frac{1}{n_0}\sum_{j:y_j=y_i}\log e^{-\alpha(\Scos_{ij}-\lambda)}]\vartriangleright \text{Jensen's inequality} \\
&= \sum_{i=1}^{n}\frac{1}{n_0}[\sum_{j:y_j=y_i}-(\Scos_{ij}-\lambda)]\\
&\ceq -\sum_{i=1}^{n}\frac{1}{n_0}\sum_{y_j=y_i}\Scos_{ij}
\end{split}
\end{align}
where $\ceq$ stands for equal to, up to an additive constant. For $\mathcal{L}_{MS}^-$ we can write:
\begin{align}\label{eqs2}
\begin{split}
\mathcal{L}_{MS}^-&=\sum_{i=1}^{n}\frac{1}{\beta}\log [1+\sum_{j:y_j\neq y_i}e^{\beta(\Scos_{ij}-\lambda)}] \\
&\geq \sum_{i=1}^{n}\frac{1}{\beta}\log [\sum_{j:y_j\neq y_i}e^{\beta(\Scos_{ij}-\lambda)}] \\
&\cgeq \sum_{i=1}^{n}\frac{1}{\beta}[\frac{1}{n_0(C-1)}\sum_{j:y_j\neq y_i}\log e^{\beta(\Scos_{ij}-\lambda)}] \\
&\quad \vartriangleright \text{Jensen's inequality} \\
&= \sum_{i=1}^{n}\frac{1}{n_0(C-1)}\sum_{j:y_j\neq y_i}\Scos_{ij}
\end{split}
\end{align}
According to Eq~(\ref{eqs1}) and Eq~(\ref{eqs2}), we have:
\begin{align}\label{eqs3}
 \mathcal{L}_{MS} \cgeq \sum_{i=1}^n\big\{-\frac{1}{n_0}\sum_{j:y_j=y_i}\Scos_{ij}+\frac{1}{(C-1)n_0}\sum_{j:y_j\neq y_i} \Scos_{ij}\big\}
\end{align}

Now we consider $\mathcal{L}_{Gen-Bin}$. Firstly, it can be written:
\begin{align}\label{eqs4}
\begin{split}
\mathcal{L}_{Gen-Bin}&\ceq\sum_{i=1}^n\big\{-\log p(\zi|y=y_i)\\
&+\frac{1}{C-1}\sum_{c=1,c\neq y_i}^C\log p(\zi|y=c)\big\}
\end{split}
\end{align}
For convenience, we denote the features of data samples whose labels are $c$ as $\{\z_{c_i}\}_{i=1}^{n_0}$. For the first part in the right hand of Eq~(\ref{eqs4}), we have:
\begin{align}\label{eqs5}
\begin{split}
&\sum_{i=1}^n-\log p(\zi|y=y_i)  \\
\ceq&\frac{1}{2}\sum_{i=1}^n\|\zi-\bmu_c^{\mathcal{D}} \|_2^2 \quad \vartriangleright p(\z|y=c)=\mathcal{N}(\z|\bmu_c^{\mathcal{D}},\mathbf{I})  \\
=&\frac{1}{2}\sum_{c=1}^C\sum_{i=1}^{n_0}\|\z_{c_i}-\bmu_c^{\mathcal{D}} \|_2^2  \\
=&\frac{1}{2}\sum_{c=1}^C\sum_{i=1}^{n_0}\big\{ \|\z_{c_i}\|_2^2-2\z_{c_i}^{\mathrm{T}}\bmu_c^{\mathcal{D}}+\|\bmu_c^{\mathcal{D}}\|_2^2 \big\} \\
\ceq&\frac{1}{2}\sum_{c=1}^C\big\{\sum_{i=1}^{n_0}-2n_0\|\bmu_c^{\mathcal{D}}\|_2^2 +n_0\|\bmu_c^{\mathcal{D}}\|_2^2 \big\}  \quad \vartriangleright \|\z\|_2^2=1 \\
=&\frac{1}{2}\sum_{c=1}^C\sum_{i=1}^{n_0}-n_0\|\bmu_c^{\mathcal{D}}\|_2^2 \\
=&\frac{1}{2}\sum_{c=1}^C\sum_{i=1}^{n_0}\sum_{j=1}^{n_0}-\frac{1}{n_0}\z_{c_i}^{\mathrm{T}}\z_{c_j}\\
=&-\sum_{i=1}^n\sum_{j:y_j=y_i} \frac{1}{2n_0}\Scos_{ij}
\end{split}
\end{align}
Keep in mind that the mean of class c $\bmu_c^{\mathcal{D}}=\frac{1}{n_0}\sum_{i=1}^{n_0}\z_{c_i}$. For the second part in the right hand of Eq~(\ref{eqs4}), we have:
\begin{align}\label{eqs6}
\begin{split}
&\sum_{i=1}^n\sum_{c=1,c\neq y_i}^C\log p(\zi|y=c)\\
=&\frac{1}{2}\sum_{i=1}^n\sum_{c=1,c\neq y_i}^C-\|\z_{i}-\bmu_c^{\mathcal{D}} \|_2^2 \\
=&\frac{1}{2}\sum_{i=1}^n\sum_{c=1,c\neq y_i}^C\big\{-\|\z_{i}\|_2^2+2\z_{i}^{\mathrm{T}}\bmu_c^{\mathcal{D}}-\|\bmu_c^{\mathcal{D}}\|_2^2\big\} \\
\ceq&\frac{1}{2} \sum_{i=1}^n\sum_{c=1,c\neq y_i}^C2\z_{i}^{\mathrm{T}}\bmu_c^{\mathcal{D}}-(C-1)n_0\sum_{c=1}^C\|\bmu_c^{\mathcal{D}}\|_2^2 \vartriangleright\|\z\|_2^2=1  \\
=&\frac{1}{2} \sum_{i=1}^n\sum_{j:y_j\neq y_i}^C\frac{2}{n_0}\z_{i}^{\mathrm{T}}\z_{j}-\frac{C-1}{n_0}\sum_{c=1}^C\sum_{i=1}^{n_0}\sum_{j=1}^{n_0}\z_{c_i}^{\mathrm{T}}\z_{c_j} \\
=&\sum_{i=1}^n\big\{\sum_{j:y_j\neq y_i} \frac{1}{n_0}\Scos_{ij}-\sum_{j:y_j=y_i} \frac{C-1}{2n_0}\Scos_{ij}\big\}
\end{split}
\end{align}
According to Eq~(\ref{eqs5}) and Eq~(\ref{eqs6}), we have:
\begin{align}\label{eqs7}
\mathcal{L}_{Gen-Bin}\ceq \sum_{i=1}^n\big\{-\frac{1}{n_0}\sum_{j:y_j=y_i}\Scos_{ij}+\frac{1}{(C-1)n_0}\sum_{j:y_j\neq y_i} \Scos_{ij}\big\}
\end{align}
According to Eq~(\ref{eqs3}) and Eq~(\ref{eqs7}), we can obtain:
\begin{align}
\mathcal{L}_{MS}\cgeq \mathcal{L}_{Gen-Bin}
\end{align}
\end{proof}








\end{document}


==> no.tex <==
%\documentclass[conference]{IEEEtran}
\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage[ruled ,linesnumbered, algo2e]{algorithm2e}

\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{times}
\usepackage{soul}
\usepackage{url}
\usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{amstex}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}
\urlstyle{same}
\usepackage{bm}
\usepackage{mathtools}
% the following package is optional:
%\usepackage{latexsym}
\usepackage{color}
\usepackage{amsfonts} % Use the postscript times font!
\usepackage{amsmath}
%\usepackage{soul}
\usepackage{url}
%\usepackage[hidelinks]{hyperref}
\usepackage[utf8]{inputenc}
%\usepackage[small]{caption}
\usepackage[switch]{lineno}

%\def\propositionautorefname{Proposition}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subfig}
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{newfloat}
\usepackage{listings}
\usepackage{amssymb}

\usepackage{enumerate}
\usepackage{mathtools}
\usepackage{booktabs}
\usepackage{makecell}
\usepackage{bbding}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\begin{document}
\title{Mutual Information Rebalancing for Online Class-Incremental Learning}




\author{\IEEEauthorblockN{Anonymous Authors}}
\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
%\newcommand{\cite}[1]{\citeauthor{#1} \shortcitep{#1}} 
%\newcommand{\cite}{\cite} 



% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\def\memory{\mathcal{M}}
\def\newbatch{\mathcal{B}_n}
\def\replaybatch{\mathcal{B}_r}
\def\tt{\bm \theta}
\def\x{\bm x}
\def\logit{\bm o}
\def\z{\bm z}
\def\y{\bm y}
\def\t{\bm t}
\def\c{\bm c}
\def\p{\bm p}
\def\haty{\hat{\bm y}}
%\newcommand{\Scos}{S^{\text{cos}}}
\newcommand{\Scos}{S}
\def\xi{{\bm x}_i}
\def\zi{{\bm z}_i}
\def\yi{{\bm y}_i}
\def\yc{{\bm y}_c}
\def\bmu{{\boldsymbol{\mu}}}
\def\D{\mathcal{D}}
\newcommand{\ceq}{\stackrel{\mathclap{\normalfont\mbox{c}}}{=}}
\newcommand{\capprox}{\stackrel{\mathclap{\normalfont\mbox{c}}}{\approx}}
\newcommand{\cleq}{\stackrel{\mathclap{\normalfont\mbox{c}}}{\leq}}
\newcommand{\cgeq}{\stackrel{\mathclap{\normalfont\mbox{c}}}{\geq}}

\maketitle
\begin{abstract}
When learning tasks sequentially, \emph{artificial neural networks} (ANNs) suffer from the problem of \emph{catastrophic forgetting}, which becomes even severer when ANNs are required to learn new classes from online data stream without task boundaries. Currently, studies on \emph{online class-incremental learning} (OCL), intending to alleviate forgetting under this condition, have gained more and more attention. In this paper, we reveal why informative features are required for OCL and how the model can employ them to improve the performance. To directly explore the feature space, we decouple the training of feature extractor and classifier, and use \emph{deep metric learning} (DML) to learn the former. By studying the behavior of DML loss function in OCL from the perspective of \emph{mutual information} (MI), we find that the components of MI are unbalanced due to its shortsighted view of future samples, which results in the information degradation of features. For this reason, we propose a general MI rebalancing method to get informative features. However, informative features have higher variance impairing the performance of classifier. Therefore, we further propose an algorithm with variance reduction under the \emph{Nearest-Class-Mean} classifier framework for OCL. Experimental results on several benchmarks show that our method remarkably outperforms a series of state-of-the-art replay-based methods. 
\end{abstract}



\section{Introduction}
Although \emph{artificial neural networks} (ANNs) have surpassed human in many areas, they are still easy to fail in some realistic scenarios. For instance, when learning a sequential of tasks emerging over time, ANNs inevitably suffer from \emph{catastrophic forgetting} \cite{1989cataf} of past trained tasks, whereas humans inherently study in a lifelong paradigm \cite{parisireview}. To bridge the gap between ANNs and humans, \emph{continual learning} (CL) \cite{parisireview,langereview}, also referred to as \emph{lifelong learning}, which studies the ability of ANNs to both preserve mastered skills and acquire novel knowledge when facing non-i.i.d data, has become a cutting-edge field of deep learning research.

Many existing CL methods alleviate catastrophic forgetting with the aid of task identifiers. Some of them focus on \emph{task-incremental} learning \cite{3sc}, where the model can acquire task identifiers both at training and inference stage, and thus using a multi-head output layer is feasible \cite{ewc,lwf}. In this setting, the model can make predictions only within a specific task by masking heads belonging to other tasks. A tougher setting is \emph{class-incremental} \cite{3sc, icarl} learning, where task identifiers are not informed to model at inference stage. The model has to classify samples over all seen classes with a single-head output layer. However, in common class-incremental setting, usage of task identifiers during training is still permitted, which makes it possible to consolidate knowledge \cite{bic}, separate parameters \cite{rps} and adjust optimization objective \cite{icarl} for each task respectively. What's more, the model can be trained on each task several epochs to achieve a stationary minimum, thus weakening the importance of its adaptation speed to new tasks. In this paper, we focus on a more realistic and challenging setting: \emph{online class-incremental learning} (OCL) \cite{gss, mir}, also referred to as \emph{task-free continual learning} \cite{task-free, dpm}, where model learns from a non-i.i.d data stream online, without the help of task identifiers or task boundaries both at training and inference stage.

Due to the wide applicability and high reliability of Experience Replay (ER), recent works on OCL are mainly based on it. Nevertheless, studies on ER used in class-incremental setting \cite{bic, il2m, wa} attribute one of the causes of forgetting to the \emph{logits bias} problem in the softmax layer of neural network, which is to say that the logits outputted by softmax layer bias toward newly seen classes significantly. Logits bias not only hurts the performance of the model, but also makes it difficult to measure the quality of feature space since features of different classes are considered unfairly. Meanwhile, current methods with softmax classifier also neglect the importance of feature space to OCL.

For a clear and direct study on feature space, in this paper we discard previous widely-used framework which jointly trains an end-to-end network. Instead, we train a feature extractor (namely embedding network) with \emph{deep metric learning} (DML) as recent work \cite{sdc} and use a non-parameter classifier to bypass logits bias. After removing the influence of softmax classifier, we focus on this issue: \emph{what kind of features are required for OCL}.

We claim that OCL benefits from features with more information, because they bring about more knowledge sharing and minimum areas overlap. Inspired by recent work on DML \cite{unifymi}, we interpret the DML loss in OCL scenario as maximizing conditional \emph{mutual information} (MI), and show that it causes the imbalance between the two components of full MI of joint training, which further results in degraded low-entropy outputted features. With the purpose of extracting informative features and thus enhancing forward transfer, we compensate for the underestimated entropy term in the loss function. However, informative features with high entropy also have high variance, conflicting with the Nearest-Class-Mean (NCM) classifier \cite{icarl} which prefers low-variance features. In order to counteract this variance increase, we propose a variance reduction algorithm by calculating the class centers during training, and correcting their drifts before inference. Additional penalty term imposed on low correlation coefficients between means calculated at different iterations of one class also guarantee the low variance, which can be further interpreted as encouraging features to get high intra-class cross-time MI for alleviating forgetting.

In summary, our contributions are as follows:
\begin{itemize}
\item Different from recent OCL methods, we focus on the learning of feature space. We analyze the behavior of DML loss used in OCL setting, point out its tendency to output low-entropy features, and propose addressing it by rebalancing the MI to extract informative features.
\item To counteract the effect of high variance from informative features during inference, we propose an algorithm with variance reduction under the NCM framework for OCL. Experimental results show that our method remarkably outperforms other state-of-the-art OCL methods.
\end{itemize}


\section{Related Work}
\subsection{Continual Learning}
Current methods of CL can be grouped into three categories \cite{langereview}. \emph{Regularization-based} methods alleviate forgetting by imposing penalty on parameters \cite{ewc} or outputs \cite{lwf}. The former adds an additional penalty term which restricts the movement of parameters according to their importance to old knowledge, so as to adjust the plasticity of each parameter. While the latter is based on knowledge distillation to retain outputs of old samples. They usually work well in task-incremental setting but fail in class-incremental learning \cite{3sc}. \emph{Parameter isolation} methods assign distinct parts of neural networks to different tasks. The whole neural networks can either be constant \cite{packnet, pathnet} or grow in structure as the number of tasks increase \cite{pnn, dpm}. \emph{Replay-based} methods store selected samples in a memory space (referred to as Experience Replay) \cite{icarl, bic, il2m, wa} or generate pseudo samples by a generative model (referred to as Generative Replay) \cite{dgr}, and retrain the model with these samples in subsequent tasks to maintain performance on old tasks. 

\subsection{Online Class-Incremental Learning}
\cite{er} first introduces \textbf{ER} into continual learning as an effective baseline. Based on this work, several OCL methods are proposed. \textbf{MIR} \cite{mir} designs a strategy to select maximally interfered examples from memory for replaying. \textbf{GSS} \cite{gss} writes data with high divergence of gradient into memory to increase diversity of stored samples. \textbf{A-GEM} \cite{agem} projects update direction to sub-space which is at an acute angle to gradients of stored samples, so that the update direction will not interfere with previous knowledge. \textbf{ASER} \cite{aser} resorts to the notion of \emph{Shapley Value} to improve the replay memory update and sampling.  

All these works use an end-to-end network and take no account of the importance of feature space. Unlike them, our work focuses on the learning of an appropriate feature space for OCL.

\subsection{Deep Metric Learning}
DML aims to learn an embedding space, where samples with similar semantics are close to each other, and dissimilar samples are encouraged to keep away from each other \cite{ms}. Siamese network \cite{siamese} with contrastive loss is first proposed to learn the embeddings (features) of faces. From then on, many well-designed pair-based DML losses are proposed. Triplet loss \cite{triplet} constructs triplets composed of a positive sample, a negative sample and an anchor. Its purpose is to learn an embedding space where the distance between a positive pair is closer than that between a negative pair, by giving a margin. N-pairs loss \cite{npairs} improves triplet loss by taking more negative samples of an anchor into account. Lifted structure loss \cite{ls} dynamically builds triplets by mining the hardest negative pairs. Multi-similarity loss \cite{ms} is derived by fully considering three kinds of similarity: self-similarity, negative relative similarity and positive relative similarity. 

DML has already been used in class-incremental scenario by SDC \cite{sdc}, which uses triplet loss to train a feature extractor. 

\section{Preliminaries}
Class-incremental setting of continual learning is widely used in recent literature, while in this paper, we consider OCL, a more difficult and realistic scenario when the models are required to learn new classes from online and task-free data stream continually. Formally, let $\mathcal{X}\subset\mathbb{R}^d$, $\mathcal{Y}\subset\mathbb{R}^l$, $\mathcal{Z}\subset\mathbb{R}^e$ denote input space, prediction space and feature space respectively. Then the purpose of our method is to learn a mapping $f: \mathcal{X}\to\mathcal{Y}$. Usually, the mapping $f$ is a composite of a \emph{feature extractor} $f_e: \mathcal{X}\to\mathcal{Z}$, which is a neural network in most cases, and a \emph{classifier} $f_c: \mathcal{Z}\to\mathcal{Y}$, for which we have many choices such as Multi-Layer Perceptron, K-Nearest Neighbor, etc. 

Like recent works, we construct our methods based on ER. At each iteration $t$, a minibatch of data $\mathcal{B}_t^s=(\boldsymbol{X}_t, \boldsymbol{y}_t)$ from data stream $\mathcal{S}$ arrives, and another minibatch of data $\mathcal{B}_t^m$ is sampled from episodic memory. The model is trained on $\mathcal{B}_t=\mathcal{B}_t^s\cup\mathcal{B}_t^m$. In the online setting, $\mathcal{B}_t^s$ is discarded after the iteration unless it is stored in memory. The new classes from $\mathcal{S}$ emerge over time, but there is no explicit task boundaries information provided to model. At inference stage, the model should classify over all classes seen. 

Since episodic memory strategy is not the focus of our work, we use two simple strategies for memory retrieval and update. For retrieval strategy, we use \emph{random sampling} with the same weight for each stored sample. For update strategy, in order to keep the stored samples of each class in balance, we divide the memory according to the number of seen classes, and use \emph{reservoir sampling} \cite{reservoir} for each class severally.

Some recent works \cite{bic, il2m, wa} show that under class-incremental setting, when using traditional one-layer classifier with softmax activation, the outputted logits always have a strong bias towards the newly learned classes. For this reason, as shown in following experiments, non-parameter classifiers on feature space perform better in OCL tasks with the participation of episodic memory. In our work, we decouple $f_e$ and $f_c$ as some previous works \cite{icarl, sdc}, and directly train $f_e$ using DML technique. 

\section{The Mutual Information View of Feature Extractor}


\subsection{Unbalanced Components of Mutual Information}
\cite{unifymi}  interpret several DML loss as a proxy of maximizing the mutual information $\mathcal{I}(Z; Y)$ between features $Z=f_e(X)$ and labels $Y$ of inputs $X$ in $\mathcal{S}$, where $X, Y, Z$ are all random variables in space $\mathcal{X, Y, Z}$ respectively. In other words, DML loss satisfies:
\begin{equation}\label{eq1}
\mathcal{L}_{DML}\cgeq-\mathcal{I}(Z; Y)=-\mathcal{H}(Z)+\mathcal{H}(Z|Y)
\end{equation}
in which $\cgeq$ denotes upper than, up to a multiplicative and/or additive constant, and $\mathcal{H}$ denotes information entropy.

Then we generalize the MI optimization objective to OCL setting. We denote iteration number, or time, as a random variable $T$. At iteration $t$, the model can only acquire partial data and classes depending on $\mathcal{S}$, and thus the optimization objective of DML loss is conditional $\mathcal{I}(Z; Y|T=t)$. Note that the conditional dependencies of $T,X,Y$ and $Z$ can be expressed as a simple Bayesian network \cite{bn} $T\to Y \to X \to Z$, so we have $\mathcal{H}(Z|Y;T)=\mathcal{H}(Z|Y)$ and $\mathcal{H}(Z|T)\leq\mathcal{H}(Z)$. Then we consider the expectation of conditional MI during training:
\begin{equation}\label{eq2}
\begin{aligned}
\mathbb{E}_t[\mathcal{I}(Z;Y|T=t)]
=& \mathcal{I}(Z;Y|T)\\
=& \mathcal{H}(Z|T)-\mathcal{H}(Z|Y;T)\\
=&\lambda\mathcal{H}(Z)-\mathcal{H}(Z|Y),\quad\lambda\in[0, 1]
\end{aligned}
\end{equation}
in which $\lambda=1$ iff $T$ and $Z$ are independent (hardly to be satisfied in practice).

The difference between eq (\ref{eq1}) and (\ref{eq2}) indicates that common MS loss used in OCL setting underestimates the entropy of $Z$, which leads to components imbalance in MI. To figure out how unbalanced MI affects the learning of feature extractor, we investigate the distribution of features with varying weight coefficients of $\mathcal{H}(Z)$.

\begin{proposition}\label{prop1}
Suppose feature $Z\in\mathbb{S}^{e-1}$ and label $Y\in\mathbb{Z}_+$ are two random variables. When function $\lambda\mathcal{H}(Z)-\mathcal{H}(Z|Y)$ achieves its maximum, the  distributions of features satisfy:
\begin{itemize}
\item Features of different classes distribute in nonoverlapping areas of $ \mathbb{S}^{e-1}$;
\item Random variable $Z$ obeys \\
\quad\textbf{a)} distribution in a zero measure set on $\mathbb{S}^{e-1}$;\\
\textbf{b)} arbitrary distribution;\\
\textbf{c)} uniform distribution, if\\
\quad\textbf{a)} $0<\lambda<1$; \textbf{b)} $\lambda=1$; \textbf{c)} $\lambda>1$. 
\end{itemize}
\end{proposition}
See Appendix for proof.

The first property guarantees that the features of different classes are separable whatever $\lambda$ is, while the second shows that when $\mathcal{H}(Z)$ is underestimated, or namely $\lambda<1$ in eq (\ref{eq2}), the distribution of features tends to shrink to a zero measure set, which leads to low-information (low-entropy) outputs. This kind of feature is welcome in common OCL methods (especially when the zero measure set is several points), since it does not violate the principle that putting features of the same class together and pushing those of different classes away to make the feature separability. 

However, we must point out that, as the first property indicates, dispersity and separability are not incompatible. When continually learning, the model should not only perform well on current task, but also learn transferable knowledge for subsequent unseen classes (known as forward transfer), so that the underlying knowledge can be shared among classes, or in other words, the parameters arrive at a potential low-loss area of future tasks. On the contrary, if the model only learns specialized knowledge which is necessary to current task without any redundant information, the model will have to learn knowledge of future tasks from scratch, resulting in an abrupter alteration of parameter minimum point, thus interfering learned knowledge. 


\subsection{Mutual Information Rebalancing (MIRe)}
In order to compensate for this underestimation, we modified the original loss function by adding a pair-based estimation of $\mathcal{H}(Z|T=t)$ at each iteration $t$. To be more specific, we estimate the distribution $p(Z|T=t)$ using kernel density estimation with von Mises-Fisher (vMF) kernel:
\[\widehat{p}(Z=f_e(\boldsymbol{x}_i)|T=t)=\frac{1}{Z_{vMF}}\mathbb{E}_{\boldsymbol{x}_j\in\mathcal{B}_t}[e^{\delta  f_e(\boldsymbol{x}_i)^\top f_e(\boldsymbol{x}_j)}],\delta >0\]
where $Z_{vMF}$ is the normalization constant of vMF distribution. 

Then with the Monte Carlo method:
\begin{equation}\label{eq3}
\begin{aligned}
\widehat{\mathcal{H}}(Z|T=t)&\\
\ceq -\mathbb{E}_{\boldsymbol{x}_i\in\mathcal{B}_t}&[\log\mathbb{E}_{\boldsymbol{x}_j\in\mathcal{B}_t}[e^{\delta  f_e(\boldsymbol{x}_i)^\top f_e(\boldsymbol{x}_j)}]],\ \delta >0
\end{aligned}
\end{equation}


In combination with the entropy estimation term, the DML loss function is modified as:
\begin{equation}\label{eq4}
\mathcal{L}_{MIRe}(\mathcal{B}_t)\triangleq\mathcal{L}_{DML}(\mathcal{B}_t) - \alpha\widehat{\mathcal{H}}(Z|T=t),\quad \alpha>0
\end{equation}

In this paper, we use Multi-similarity (MS) loss \cite{ms}, one of the state-of-the-art metric learning methods as a representative of DML.
\section{Classifier with Variance Reduction}
Given a well trained feature extractor, we now require a suitable classifier to propagate the information from episodic memory to make inference. Typically, Nearest-Class-Mean (NCM) classifier is widely used in CL introduced into this field by \cite{icarl}. Let $\mathcal{M}_c$ denote the subset of episodic memory $\mathcal{M}$, where all samples belong to class $c$. During inference, the prediction for input $\boldsymbol{x}^*$ is:
\begin{equation}
\label{ncm}
y^*=\mathop{\arg\min}_{c} ||f_e(\boldsymbol{x}^*)-\boldsymbol{m}_c ||_2
\end{equation}
in which $\boldsymbol{m}_c=\frac{1}{|\mathcal{M}_c|}\sum_{\boldsymbol{x}\in\mathcal{M}_c}f_e(\boldsymbol{x})$ is the approximate class mean of class $c$.

By simply replacing the last softmax layer with NCM classifier at inference stage, current state-of-the-art OCL methods can bypass the logits bias problem and thus get a performance gain by a large margin.

\subsection{Preference conflict between $f_e$ and $f_c$}
In NCM classifier, the mean of each distribution is an estimation $\boldsymbol{m}_c$ given by stored samples, instead of the true mean value. The variance of the estimation has a significant impact on the precision of NCM classifier. For simplicity, we suppose the dimensions of feature $Z$ are independent of each other, and denote the variance and mean of $Z_i|Y=c$ as $(\boldsymbol{\sigma}_c^i)^2$ and $\boldsymbol{\mu}_c^i$. Then according to the Central Limit Theorem, the $i$-th dimension of $\boldsymbol{m}_c$ obeys a Gaussian distribution: \[\boldsymbol{m}_c^i\sim\mathcal{N}(\boldsymbol{\mu}_c^i, \frac{(\boldsymbol{\sigma}_c^i)^2}{|\mathcal{M}_c|})\]

The performance of NCM classifier is limited by two factors. First, the number of stored samples $|\mathcal{M}_c|$ is restricted. Second, as in Section 4, we encourage the features distribute uniformly, and we empirically find that it results in an increase in the variance of features in each class. This reveals that there is a conflict between $f_e$ and $f_c$: $f_e$ prefers features that are informative and have a wide distribution thus promoting knowledge sharing, while $f_c$ prefers highly-centralized features for precise estimation of class means. For this reason, it is inadvisable to directly use features from $f_e$ for $f_c$ like NCM classifier.


\subsection{Prototype Maintenance \& Drift Correction}
\begin{figure}[t]
\centering
\includegraphics[width=8cm]{fig/var.pdf}
\caption{For each of the first 5 classes in 20-task Split CIFAR-100, we calculate its element-wise variance of features with validation set after each task, and average it over dimensions. The feature extractor is trained with $\mathcal{L}_{MIRe}$.}
\label{var}
\end{figure}
An intuitive way to reduce variance is to calculate the class means during training, as the samples seen by the model at training stage are much more than those in episodic memory. But as \cite{sdc} point out, with the training of subsequent tasks, the features extracted by the extractor will change, and the prototypes calculated in the previous iterations cannot accurately represent the actual class means in the subsequent iterations. This phenomenon is called \emph{semantic drift} \cite{sdc} or \emph{feature drift} \cite{xbm} of the prototypes.

\cite{sdc} solve this problem by estimating and compensating for the drifts with new samples. With the help of episodic memory, we can simplify this process by using stored samples to estimate them. For all notations used following, the superscript $i$ stands for the $i$-th dimension. At iteration $t$, we suppose that we have an estimation of current $\boldsymbol{\mu}_c^{i,t}$ with negligible variance, and we denote it as $\boldsymbol{p}_c^{i,t}$. And then, let $\boldsymbol{m}_c^{i,t}$ and $\boldsymbol{m}_c^{i,t'}$ denote the estimation of $\boldsymbol{\mu}_c^{i,t}$ made by stored samples at iteration $t$ and inference time $t'>t$. We can compensate the semantic drift by:
\begin{equation}\label{sdc}
\widetilde{\boldsymbol{\mu}}_c^{i,t'}\triangleq\boldsymbol{p}_c^{i,t}-\boldsymbol{m}_c^{i,t}+\boldsymbol{m}_c^{i,t'}
\end{equation}
And then we can make predictions as eq (\ref{ncm}) with $\widetilde{\boldsymbol{\mu}}_c^{i,t'}$ as the approximate class mean instead. $\widetilde{\boldsymbol{\mu}}_c^{i,t'}$ is an unbiased estimation with variance:
\[D(\widetilde{\boldsymbol{\mu}}_c^{i,t'})=\frac{(\boldsymbol{\sigma}_c^{i,t})^2+(\boldsymbol{\sigma}_c^{i,t'})^2-2\boldsymbol{\rho}_c^{i,t,t'}\boldsymbol{\sigma}_c^{i,t}\boldsymbol{\sigma}_c^{i,t'}}{|\mathcal{M}_c|}\]
in which $\boldsymbol{\rho}_c^{i,t,t'}$ is the correlation coefficient (CC) between $\boldsymbol{m}_c^{i,t}$ and $\boldsymbol{m}_c^{i,t'}$.

Compared with NCM classifier directly using $\boldsymbol{m}_c^{i,t'}$ as a class mean, $D(\widetilde{\boldsymbol{\mu}}_c^{i,t'})$ is lower than $D(\boldsymbol{m}_c^{i,t'})$ iff $\boldsymbol{\sigma}_c^{i,t}<2\boldsymbol{\rho}_c^{i,t,t'}\boldsymbol{\sigma}_c^{i,t'}$. As in Figure \ref{var}, we empirically find that $\boldsymbol{\sigma}_c^{i,t'}$ is higher than $\boldsymbol{\sigma}_c^{i,t}$ in most cases. Therefore, we can restrict $D(\widetilde{\boldsymbol{\mu}}_c^{i,t'})$ by increasing $\boldsymbol{\rho}_c^{i,t,t'}$ to achieve lower variance. 



To this end, we modify the process of drift correction under OCL setting, where we don't have an exact iteration $t$ instructed by task boundaries to calculate $\boldsymbol{m}_c^{i,t}$ and $\boldsymbol{\rho}_c^{i,t,t'}$. For each sample $\boldsymbol{x}$, we define the iteration $t$ in eq (\ref{sdc}) as the iteration when $\boldsymbol{x}$ appears in $\mathcal{B}^s_t$. If $\boldsymbol{x}$ is stored in memory, we also store its feature $\boldsymbol{z}$ of the moment. We calculate the CC as follows:
\begin{equation}\label{cc}
\widehat{\boldsymbol{\rho}}_c^{i,{t'}}=\frac{\sum_{(\boldsymbol{x},\boldsymbol{z})\in\mathcal{M}^{t'}_c}{(f_e^i(\boldsymbol{x})}-\boldsymbol{m}_c^i)(\boldsymbol{z}^i-\overline{\boldsymbol{z}}^i_c)}{\sqrt{\sum_{\boldsymbol{x}\in\mathcal{M}^{t'}_c}{(f_e^i(\boldsymbol{x})}-\boldsymbol{m}_c^i)^2}\sqrt{\sum_{\boldsymbol{z}\in\mathcal{M}^{t'}_c}{(\boldsymbol{z}^i-\overline{\boldsymbol{z}}^i_c)^2}}}
\end{equation}
in which $\mathcal{M}^{t'}_c$ is a subset of $\mathcal{M}_c$ randomly selected at iteration ${t'}$ (for efficiency) and $\overline{\boldsymbol{z}}^i_c=\frac{1}{|\mathcal{M}^{t'}_c|}\sum_{\boldsymbol{z}^i\in\mathcal{M}^{t'}_c}{\boldsymbol{z}^i}$. 

In accordance with the CC, at inference stage, we calculate the $\boldsymbol{m}_c^{i,t}$ in eq (\ref{sdc}) as $\overline{\boldsymbol{z}}^i_c$. As for ${\boldsymbol{p}}_c^{i,t}$, we cannot get the whole training set in OCL setting, so we calculate it by maintaining a momentum-updated prototype: 
\begin{equation}\label{proto}
{\boldsymbol{p}}_c^{i,t}\triangleq\gamma{\boldsymbol{p}}_c^{i,t-1}+\frac{(1-\gamma)}{\mathcal{B}^s_{t,c}}\sum_{x\in\mathcal{B}^s_{t,c}}{f_e^i(\boldsymbol{x})}
\end{equation}
in which $\mathcal{B}^s_{t,c}$ is the subset of $\mathcal{B}^s_{t}$ of class $c$. The prototypes are projected to the unit hypersphere after update. 

Then, eq (\ref{eq4}) is modified as:
\begin{equation}\label{eq5}
\mathcal{L}_{MIRe++}(\mathcal{B}_t, \mathcal{M})\triangleq
\mathcal{L}_{MIRe}(\mathcal{B}_t)-\beta\sum_{i,c}\widehat{\boldsymbol{\rho}}_c^{i,t},\ \beta>0
\end{equation}

The operation of placing CC penalty can also be explained in the framework of MI. When training with new classes, the learned features of old classes will be interfered, and hence some information will be forgotten. Formally speaking, let random variable $Z^{t}_c$ denote a feature of class $c$ at iteration $t$. After iteration $t'>t$, the feature becomes $Z^{t'}_c$, and the MI between these two random variables $\mathcal{I}(Z^{t}_c;Z^{t'}_c)$ can be interpreted as the remembered information of $Z^{t}_c$. We simplify this MI by assuming $Z^{t}_c$ and $Z^{t'}_c$ are multivariate Gaussian distribution, and their dimensions are independent of each other. Then we have:
\[\mathcal{I}(Z^{t}_c;Z^{t'}_c)=-\sum_{i}{\frac{1}{2}\log(1-(\boldsymbol{\rho}_c^{i,t,t'})^2)}\]
This equation demonstrates that maximizing the CC is equivalent to maximizing the \emph{intra-class cross-time MI} $\mathcal{I}(Z^{t}_c;Z^{t'}_c)$ under a series of ideal hypothesises.
\section{Experimental Results}
\begin{table*}[htb]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{p{2.2cm}<{\centering}|p{1.2cm}<{\centering}p{1.2cm}<{\centering}|p{1.2cm}<{\centering}p{1.2cm}<{\centering}|p{1.2cm}<{\centering}p{1.2cm}<{\centering}|p{1.2cm}<{\centering}p{1.2cm}<{\centering}|p{1.2cm}<{\centering}p{1.2cm}<{\centering}}
\toprule[1.0pt]
Methods &\multicolumn{2}{c}{\tabincell{c}{Split CIFAR-10 \\(5-task)}} &\multicolumn{2}{c}{\tabincell{c}{Split CIFAR-100 \\(10-task)}} &\multicolumn{2}{c}{\tabincell{c}{Split CIFAR-100 \\(20-task)}}&\multicolumn{2}{c}{\tabincell{c}{Split MiniImageNet \\(10-task)}}&\multicolumn{2}{c}{\tabincell{c}{Split MiniImageNet \\(20-task)}}\\  
\specialrule{0em}{1pt}{1pt}
\hline
\specialrule{0em}{1pt}{1pt}
NCM&w/o&w/&w/o&w/&w/o&w/&w/o&w/&w/o&w/\\
\hline \hline 

\specialrule{0em}{1pt}{1pt}
ER &24.36$_{\pm0.89}$&31.31$_{\pm2.17}$& 9.84$_{\pm0.36}$&14.87$_{\pm0.37}$&6.26$_{\pm0.52}$&12.33$_{\pm0.31}$&7.73$_{\pm0.34}$&13.32$_{\pm0.42}$&6.27$_{\pm0.27}$&12.35$_{\pm0.51}$\\
A-GEM  &18.32$_{\pm0.18}$&28.15$_{\pm1.44}$
&6.38$_{\pm0.15}$&10.73$_{\pm0.42}$
&3.52$_{\pm0.12}$&8.07$_{\pm0.44}$
&4.14$_{\pm0.18}$&8.15$_{\pm0.36}$
&3.25$_{\pm0.32}$&6.23$_{\pm0.49}$\\
GSS-Greedy  &23.41$_{\pm1.11}$&29.57$_{\pm1.43}$
&9.98$_{\pm0.20}$&11.35$_{\pm0.79}$
&5.89$_{\pm0.36}$&10.57$_{\pm0.41}$
&7.98$_{\pm0.89}$&12.52$_{\pm0.69}$
&5.57$_{\pm0.47}$&12.05$_{\pm0.63}$\\
MIR &24.18$_{\pm0.77}$&31.08$_{\pm1.65}$
&9.90$_{\pm0.49}$&14.37$_{\pm0.32}$
&6.20$_{\pm0.57}$&11.48$_{\pm0.42}$
&7.81$_{\pm0.28}$&14.23$_{\pm0.50}$
&5.98$_{\pm0.47}$&12.71$_{\pm0.41}$\\

ASER$_{\mu}$   &30.97$_{\pm1.03}$&35.42$_{\pm1.06}$
& 12.33$_{\pm0.64}$& 18.29$_{\pm0.51}$
&8.83$_{\pm0.55}$&15.79$_{\pm0.53}$
& 10.87$_{\pm0.54}$&13.64$_{\pm0.92}$
&8.27$_{\pm0.61}$&12.98$_{\pm0.65}$\\
\specialrule{0em}{1pt}{1pt}
\hline 

\specialrule{0em}{1pt}{1pt}
MIRe (ours)  &\multicolumn{2}{c}{51.47$_{\pm1.15}$}&\multicolumn{2}{c}{18.03$_{\pm0.35}$}&\multicolumn{2}{c}{18.08$_{\pm0.33}$}&\multicolumn{2}{c}{14.39$_{\pm0.40}$}&\multicolumn{2}{c}{14.26$_{\pm0.38}$}\\

MIRe++ (ours)
&\multicolumn{2}{c}{\textbf{52.22$_\mathbf{\pm1.01}$}}
&\multicolumn{2}{c}{\textbf{19.92$_\mathbf{\pm0.48}$}}
&\multicolumn{2}{c}{\textbf{19.37$_\mathbf{\pm0.26}$}}
&\multicolumn{2}{c}{\textbf{16.62$_\mathbf{\pm0.31}$}}
&\multicolumn{2}{c}{\textbf{15.41$_\mathbf{\pm0.42}$}}\\  
\specialrule{0em}{1pt}{1pt}
\hline
\specialrule{0em}{1pt}{1pt}
fine-tune  &\multicolumn{2}{c}{18.63$_{\pm0.15}$}& \multicolumn{2}{c}{6.20$_{\pm0.32}$} &\multicolumn{2}{c}{3.67$_{\pm0.11}$} &\multicolumn{2}{c}{4.28$_{\pm0.24}$}&\multicolumn{2}{c}{3.20$_{\pm0.15}$}\\
i.i.d. online  &\multicolumn{2}{c}{62.76$_{\pm1.68}$} &\multicolumn{2}{c}{20.22$_{\pm0.66}$}& \multicolumn{2}{c}{20.22$_{\pm0.66}$ }&\multicolumn{2}{c}{18.13$_{\pm0.66}$}&\multicolumn{2}{c}{18.13$_{\pm0.66}$}\\
i.i.d. offline  &\multicolumn{2}{c}{79.47$_{\pm0.37}$}&\multicolumn{2}{c}{45.94$_{\pm0.28}$}& \multicolumn{2}{c}{45.94$_{\pm0.28}$}&\multicolumn{2}{c}{38.80$_{\pm0.55}$}&\multicolumn{2}{c}{38.80$_{\pm0.55}$} \\
\bottomrule[1.0pt]
\end{tabular}
}
\end{center}
\caption{Average Accuracy of 10 runs. For each baseline, we report two results with and without NCM classifier.}
\label{table1}
\end{table*}


\begin{table}[htb]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{p{1.5cm}<{\centering}p{1.0cm}<{\centering}p{1.0cm}<{\centering}p{1.0cm}<{\centering}p{1.5cm}<{\centering}p{1.5cm}<{\centering}}
\toprule[1.0pt]
Methods &{\tabincell{c}{Split \\ CIFAR-10 \\(5-task)}} &{\tabincell{c}{Split \\ CIFAR-100 \\(10-task)}} &{\tabincell{c}{Split \\ CIFAR-100 \\(20-task)}}&{\tabincell{c}{Split\\MiniImageNet \\(10-task)}}&{\tabincell{c}{Split\\MiniImageNet \\(20-task)}}\\  
\specialrule{0em}{1pt}{1pt}

\hline \hline 
\specialrule{0em}{1pt}{1pt}


ER
&59.60$_{\pm2.13}$&41.97$_{\pm0.84}$&54.10$_{\pm0.73}$&34.34$_{\pm0.97}$&45.91$_{\pm0.84}$\\
A-GEM
&66.74$_{\pm1.19}$
&43.55$_{\pm1.09}$&58.13$_{\pm0.93}$
&35.77$_{\pm0.92}$&48.34$_{\pm1.41}$\\
GSS-Greedy
&67.06$_{\pm0.64}$
&40.18$_{\pm0.95}$&54.21$_{\pm0.94}$
&34.07$_{\pm1.07}$&47.18$_{\pm1.30}$\\
MIR
&61.04$_{\pm1.24}$
&42.26$_{\pm0.85}$&54.01$_{\pm1.06}$
&35.57$_{\pm1.13}$&45.87$_{\pm1.33}$\\

ASER$_{\mu}$&55.34$_{\pm1.13}$&35.42$_{\pm0.91}$&56.48$_{\pm0.82}$&45.49$_{\pm0.95}$&46.99$_{\pm0.95}$\\
\specialrule{0em}{1pt}{1pt}
\hline
\specialrule{0em}{1pt}{1pt}
MIRe 
&{40.22$_{\pm1.63}$}
&\textbf{22.12$_{\pm0.53}$}
&\textbf{24.22$_{\pm0.55}$}
&\textbf{13.73$_{\pm0.47}$}
&\textbf{15.53$_{\pm0.47}$}\\ 
MIRe++ 
&\textbf{39.09$_{\pm1.35}$}
&{26.20$_{\pm0.61}$}
&{30.15$_{\pm0.57}$}
&{19.97$_{\pm0.51}$}
&{21.66$_{\pm0.49}$}\\  
\specialrule{0em}{1pt}{1pt}
\hline
\specialrule{0em}{1pt}{1pt}
fine-tune
&{85.60$_{\pm0.57}$}&{51.19$_{\pm0.93}$}&{65.37$_{\pm0.76}$}&{41.23$_{\pm0.85}$}&{52.95$_{\pm0.96}$}
\\
\bottomrule[1.0pt]
\end{tabular}
}
\end{center}
\caption{Average Forgetting of 10 runs.}
\label{table2}
\end{table}

\subsection{Experiment Setup}

\subsubsection{Datasets}
We evaluate our methods on three image classification datasets widely used in OCL literature \cite{mir, aser}: \textbf{Split CIFAR-10}, \textbf{Split CIFAR-100} and \textbf{Split MiniImageNet}. They respectively split CIFAR-10 \cite{cifar}, CIFAR-100 \cite{cifar} and MiniImageNet \cite{mini} dataset into subsets with nonoverlapping classes. Split CIFAR-10 consists of 5 tasks, each of which contains samples from 2 classes. Likewise, the 100 classes of CIFAR-100 and MiniImageNet are separated into 10 or 20 tasks. Although we construct the data stream by explicitly assigning different classes to disjoint tasks, we still follow the restriction of OCL that task boundaries are not informed during training and inference. The minibatch size of new data is fixed to 10 for all datasets and methods.
\subsubsection{Baselines}
\begin{figure}[t]
\centering
\includegraphics[width=9cm]{fig/fig_pertask.pdf}
\caption{Average Accuracy on already learned task during training.}
\label{pertask}
\end{figure}
We compare our methods with a series of state-of-the-art OCL baselines mentioned in Section 2.2: \textbf{ER} \cite{er}, \textbf{A-GEM} \cite{agem}, \textbf{GSS} \cite{gss}, \textbf{MIR} \cite{mir}, and \textbf{ASER} \cite{aser}. For methods that have multiple variants, we choose the one which performs best in the original paper, i.e. GSS-Greedy for GSS and ASER$_\mu$ for ASER. For a direct comparison of the effectiveness of feature extractor, we report results under two settings for each baseline to isolate the influence (especially logits bias) of classifier: one is consistent with its original paper, and the other one enhances the method by replacing the last fully-connected layer with NCM classifier. In addition, we also provide some non-CL results: \textbf{fine-tune} trains the model without any OCL techniques; \textbf{iid-online} and \textbf{iid-offline} shuffle all training data to get an i.i.d. data stream and train the model for 1 and 5 epochs respectively. 
\subsubsection{Implementation details}
We report the result of proposed \textbf{MIRe++}, which trains the feature extractor with $\mathcal{L}_{MIRe++}$ and infers with the variance-reduced classifier. For a fairly comparison between feature extractors, we also report \textbf{MIRe}, a semi-finished method of MIRe++, which trains with $\mathcal{L}_{MIRe}$ and infers with NCM classifier. Following the baselines, we use a reduced Resnet-18 \cite{resnet} without the last fully-connected layer as feature extractor. We project the extracted features to 128-dimension space by a Multi-Layer Perceptron head with 2 layers before calculating the MS loss and entropy, while the raw features are still used for classification. The memory space of our methods is 200 for Split CIFAR-10 and 500 for other datasets. Note that we use a relatively small budget to mimic a practical setting. Our methods need to store features, which take up about the same size of space as 31.3, 78.1 and 45.4 samples on the three datasets respectively. For a fair comparison, we store 240, 600 and 550 samples (more than 231.3, 578.1 and 545.4) for other ER-based baselines. All models are optimized by SGD. The single-head evaluation is always used during inference. 

Since DML benefits from a larger minibatch size \cite{xbm}, we select 100 samples from memory for replay each iteration, and duplicate the number of samples by combining the minibatch with its augmentation. To exhibit the general applicability of our methods, we do not tune the hyperparameters of MS loss, but directly employ its official implementation. More details about hyperparameter selection are provided in Appendix.% with $\alpha_{ms}=2$, $\beta_{ms}=50$ and $\lambda=0.5$.
\subsubsection{Metrics}
For evaluation, we use \textbf{Average Accuracy} and \textbf{Average Forgetting} as in previous work \cite{tiny}. We report results averaged over 10 runs, as well as their 95\% confidence intervals.

\subsection{Performance Evaluation}

Firstly, we compare our methods with other baselines with their original softmax classifier structure. As in Table \ref{table1} and Table \ref{table2}, both of our methods outperform other baselines by a large margin in Average Accuracy and Forgetting. We also fairly compare the feature extractor of all methods by using NCM classifier uniformly. Despite the large performance gains gotten from NCM classifier by all baselines, our feature extractor MIRe has a higher accuracy than other baselines on all datasets except 10-task Split CIFAR-100, where MIRe has a similar performance with ASER$_\mu$+NCM. This indicates that the features extracted by MIRe indeed meet the requirements of OCL. Moreover, by improving the classifier with variance reduction technique, MIRe++ classifies more accurately than MIRe and outperforms all state-of-the-art baselines. Figure \ref{pertask} also illustrates that our methods perform stably during the whole training process. 

As shown in Table \ref{table2}, proposed MIRe and MIRe++ forget less than other baselines. MIRe forgets fewer than MIRe++ on 100-class datasets, because for MIRe++, when a class has just been learned, there is little semantic drift on its prototype, so the prototype is a precise class mean, causing a high accuracy on this new class.
\subsubsection{Ablation Study}

We further study the ablation of our methods on Split CIFAR-10 and 10-task Split CIFAR-100, and summarize it in Table \ref{table3}. On Split CIFAR-100, MI rebalancing, drift correction and CC penalty can all help to alleviate catastrophic forgetting. Especially, our improved classifier with corrected prototypes performs well exclusively without MI rebalancing. While on Split CIFAR-10, MI rebalancing contributes more improvement, since the model is more tolerant of classifier variance on datasets with fewer classes. Moreover, drift correction cannot guarantee the variance to decrease, so it may have negative effect without CC penalty.
\begin{table}[t]
\begin{center}
\scalebox{0.8}{
\begin{tabular}{p{2.3cm}<{\centering}|p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}}
\toprule[1.0pt]

MI Rebalancing &$\times$&$\times$&\checkmark&\checkmark&\checkmark\\
\tabincell{c}{Prototypes \&\\ Drift Correction}&$\times$&\checkmark&$\times$&\checkmark&\checkmark\\
CC Penalty &$\times$&\checkmark&$\times$&$\times$&\checkmark\\
\specialrule{0em}{1pt}{1pt}
\hline \hline
\specialrule{0em}{1pt}{1pt}
\tabincell{c}{CIFAR-10\\ (5-task)}
&49.34$_{\pm0.83}$&49.33$_{\pm1.12}$&51.47$_{\pm1.15}$
&50.75$_{\pm0.96}$&\textbf{52.22$_\mathbf{\pm1.01}$}\\ 
\tabincell{c}{CIFAR-100\\ (10-task)}
&16.79$_{\pm0.40}$&18.27$_{\pm0.43}$&18.03$_{\pm0.35}$&19.43$_{\pm0.42}$&\textbf {19.92$_\mathbf{\pm0.48}$}\\ 
\bottomrule[1.0pt]
\end{tabular}
}
\end{center}
\caption{Ablation study of MIRe++. \checkmark and $\times$ stand for using and not using the corresponding technique respectively. We report Average Accuracy on Split datasets of 10 runs. }
\label{table3}
\end{table}
\subsection{Further Analysis}

\subsubsection{Forward transfer}

As in Section 4, we claim that MIRe aims to extract informative features, which encourages the model parameters to arrive at a potential low loss area for future classes, and thus promote knowledge sharing among classes. To verify this, we train the first task of 10-task Split CIFAR-100 for 5 epochs, and then use NCM classifier with true class means calculated with test set samples to classify the images of subsequent tasks. In other words, we let the model fulfil the remaining 9 unseen tasks with the mere knowledge of the first task. For an obvious comparison, we report the gaps of average accuracy between each unseen task and the first task. As shown in Figure \ref{fwdtsf}, MIRe reduces the accuracy gaps on all unseen tasks. These results indicate that the knowledge learned by MIRe can be transferred to subsequent tasks.
\subsubsection{Class mean estimation}
\begin{figure}[t]
\centering
\includegraphics[width=8cm]{fig/fwdtsf.pdf}
\caption{Accuracy Gap on task 2 to 10 of 10-task Split CIFAR-100 with feature extractors trained on task 1.}
\label{fwdtsf}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[width=8cm]{fig/cme.pdf}
\caption{Average Euclidean distance between true class means and estimations of all already learned tasks. MS-NCM means training the feature extractor with MS loss, and classifying with NCM classifier. }
\label{cme}
\end{figure}
As in Section 5, motivated by the claim that the NCM classifier of MIRe has higher variance, we use drift-corrected prototypes instead of class means calculated with stored samples as estimations of true class means. To verify our claim and illustrate that MIRe++ has a lower error than MIRe, we train three feature extractors on 20-task Split CIFAR-100 with MS loss, MIRe, and MIRe++ respectively. After each task, we average the Euclidean distances between true class means (calculated with test set) and the estimated means over all already learned tasks. Figure \ref{cme} shows that MIRe indeed gives a rise to higher estimation error. By comparing MIRe and MIRe++, we find that NCM classifier performs better in early tasks when each class is assigned a larger episodic memory space, since its estimations are precise enough. While as the training goes on, our corrected prototypes have a lower average error, when the memory space for each class is tiny.
\section{Conclusions}
In this work, we focus on the learning of features space in OCL. We claim that OCL needs informative features which improve knowledge sharing and forward transfer. We point out that the imbalance between components of the MI view of DML-based feature extractor causes the tendency to output low-information features, which is addressed by proposed MI rebalancing. Moreover, we indicate that classifier prefers low-variance features conflicting with the high variance of informative features. So, we further propose a variance reduction algorithm based on NCM classifier. Experimental results show that our MIRe++ outperforms other baselines. Further analysis confirms the effectiveness of our methods to improve forward transfer and class mean estimation.
\bibliographystyle{IEEEtran}
\bibliography{aaai}
\appendix

\subsection{Proof of Proposition 1}

\begin{proof}
The function $\lambda\mathcal{H}(Z)-\mathcal{H}(Z|Y)$ can be transformed into:
\[\mathcal{H}(Y)-\mathcal{H}(Y|Z) +(\lambda-1)\mathcal{H}(Z)\]
where $\mathcal{H}(Y)$ is defined by the data stream. So we only need to maximize $-\mathcal{H}(Y|Z) +(\lambda-1)\mathcal{H}(Z)$.

Firstly we have $-\mathcal{H}(Y|Z)\leq0$, where the maximum is achieved iff $Y|Z$ is one-point distribution. Or in other words, features of different classes are distributed in nonoverlapping areas.

As for $(\lambda-1)\mathcal{H}(Z)$, we discuss it in three conditions:
\begin{itemize}
    \item If $\lambda=1$, the distribution of $Z$ does not affect the function.
    \item If $0<\lambda<1$, we have $(\lambda-1)\mathcal{H}(Z) \leq 0$, where the maximum is achieved iff $Z$ is distributed in a zero measure set of $\mathbb{S}^{e-1}$.
    \item If $\lambda>1$, we have $(\lambda-1)\mathcal{H}(Z) \leq (\lambda-1)\log |\mathbb{S}^{e-1}|$, where the maximum is achieved iff $Z$ is uniformly distributed on $\mathbb{S}^{e-1}$.
\end{itemize}

Since in all of the conditions above, distribution of $Z$ is irrelevant to the distribution area of each class, the maximum conditions of $-\mathcal{H}(Y|Z)$ and $(\lambda-1)\mathcal{H}(Z)$ can be simultaneously satisfied.
\end{proof}

\subsection{Algorithm Pseudocode}
As described in the main text, we provide corresponding pseudocode of MIRe and MIRe++ at training and inference stage.
\SetKwInOut{KwOut}{Initialize}
\begin{algorithm2e}
  \SetAlgoLined
  \KwIn{Data stream $\mathcal{S}$, Learning rate $\eta$, Loss hyperparameters $\alpha$, $\beta$\\}
  \KwOut{Parameters $\theta$ of $f_e$, Episodic memory $\mathcal{M}$, Prototypes $\boldsymbol{p}$\\}
  \For{$\mathcal{B}_t^s$ in $\mathcal{S}$}{
    $\mathcal{B}_t^m\leftarrow RandomlySample(\mathcal{M})$\\
    $\mathcal{B}_t\leftarrow\mathcal{B}_t^s\cup\mathcal{B}_t^m$\\
    $\mathcal{L}\leftarrow\mathcal{L}_{MIRe}(\mathcal{B}_t)+\mathcal{L}_{MIRe}( augment(\mathcal{B}_t)$)\\
    \If{MIRe++}{
    \For{$c$ is the class which has samples in $\mathcal{M}$}{
        $\{(\boldsymbol{x}_i,\boldsymbol{z}_i)\}_i\leftarrow RandomlySample(\mathcal{M}_c)$\\
        $\rho\leftarrow$ CC between $\{f_e(x_i)\}_i$ and $\{z_i\}_i$ \tcp {as eq (7)}
        
        
        $\mathcal{L}\leftarrow\mathcal{L}-\beta\rho$
    }
    }
    $\theta\leftarrow SGD(\theta,\mathcal{L},\eta)$\\
    $Update(\mathcal{M}, \mathcal{B}_t^s, \theta)$
    \tcp {Reservoir Sampling for each class}
    $Update(\boldsymbol{p}, \mathcal{B}_t^s, \theta)$ \tcp {as eq (8)}
    }
  \caption{Training}
\end{algorithm2e}

\begin{algorithm2e}
  \SetAlgoLined
  \KwIn{Parameters $\theta$ of $f_e$, Episodic memory $\mathcal{M}$, Prototypes $\boldsymbol{p}$, Test set $\mathcal{D}_{te}$\\}
  \For{$c$ is the class which has samples in $\mathcal{M}$}  {
  $\{\boldsymbol{x}_i\}_i, \{\boldsymbol{z}_i\}_i\leftarrow\mathcal{M}_c$\\
  $\boldsymbol{m}_c\leftarrow normalize(avg_i(f_e(\boldsymbol{x}_i)))$\\
  $\overline{\boldsymbol{z}}_c \leftarrow normalize(avg_i(\boldsymbol{z}_i))$\\
  \If{MIRe++}{
  $\boldsymbol{m}_c\leftarrow normalize(\boldsymbol{p}_c-\overline{\boldsymbol{z}}_c+\boldsymbol{m}_c)$
  
  }
  \For{$\boldsymbol{x}^*\in\mathcal{D}_{te}$}{
  $y^*=\mathop{\arg\min}_{c} ||f_e(\boldsymbol{x}^*)-\boldsymbol{m}_c ||_2$
  }}
  \caption{Inference}
\end{algorithm2e}
\subsection{Hyperparameter Selection}
We tune only 3 hyperpameters of our methods: penalty weight $\alpha$ and $\beta$ in $\mathcal{L}_{MIRe++}$ and learning rate $\eta$. We select $\alpha$ and $\beta$ from \{0.001, 0.002, 0.005, 0.01, 0.02, 0.05, 0.1, 0.2, 0.5\}, and select $\eta$ from \{0.5, 0.2, 0.1, 0.05\}. As for $\delta$ in eq (3) and $\gamma$ in eq (8), we fix $\delta=5$ and $\gamma=0.99$ for all datasets. The results of hyperparameter selection are listed in Table \ref{hs}.
\begin{table}[h]
\begin{center}
\scalebox{1}{
\begin{tabular}{p{2cm}<{\centering}|p{1.5cm}<{\centering}p{1.5cm}<{\centering}p{2cm}<{\centering}}
\toprule[1.0pt]

Hyperparameter &Split CIFAR-10&Split CIFAR-100&Split MiniImageNet\\
\specialrule{0em}{1pt}{1pt}
\hline \hline
\specialrule{0em}{1pt}{1pt}
$\alpha$&0.02&0.1&0.05\\
$\beta$&0.01&0.002&0.005\\
$\eta$&0.2&0.2&0.1\\
\bottomrule[1.0pt]
\end{tabular}
}
\end{center}
\caption{Hyperparameter selection.}
\label{hs}
\end{table}
\subsection{Metrics}
\noindent Average Accuracy:
\[ACC=\frac{1}{T}\sum_{i=1}^T{a_{T,j}}\]
Average Forgetting:
\[FGT=\frac{1}{T-1}\sum_{i=1}^{T-1}{\max_{j\in[1,T-1]}a_{j,i}-a_{T,i}}\]
in which $a_{j,i}$ denotes the accuracy of task $i$ after learning task $j$.
\subsection{Applicability to Other Loss}
As we mention in Section 3, we use MS loss as a representative of DML loss. We further examine the general applicability of MIRe on Triplets loss and N-pairs loss. Results in Table \ref{AOL} indicate that MIRe is also valid for other DML losses.
\begin{table}[h]
\begin{center}
\scalebox{1}{
\begin{tabular}{p{2.5cm}<{\centering}|p{2cm}<{\centering}p{2cm}<{\centering}}
\toprule[1.0pt]

Losses &w/o MIRe&w/ MIRe\\
\specialrule{0em}{1pt}{1pt}
\hline \hline
\specialrule{0em}{1pt}{1pt}
Triplets &16.61$_{\pm0.37}$&\textbf{18.99$_\mathbf{\pm0.45}$}\\
N-pairs&13.57$_{\pm0.46}$&\textbf{14.87$_\mathbf{\pm0.50}$}\\
\bottomrule[1.0pt]
\end{tabular}
}

\end{center}
\caption{Average Accuracy on 10-task Split CIFAR-100.}
\label{AOL}
\end{table}

\end{document}

